TOTEM: TOkenized Time Series EMbeddings for General Time Series Analysis

This work studies the problem of time series analysis with generalist (or foundation) models, which are models trained across many data domains. Drawing inspiration from the widespread success of large language models, we consider the simple strategy of discretely tokenizing time series data drawn from a myriad of datasets via self-supervision, then using the fixed tokenization to solve a variety of tasks across many data domains. Canonically, time series models are either trained on a single dataset or built in a task-specific manner (e.g., a forecasting-only model), where many use patches of time as inputs to the model. As such, performant generalist, discrete representation time series models explored across many tasks are of value. Our method, TOkenized Time Series EMbeddings (TOTEM), produces such generalist time series models with minimal or no fine-tuning while exhibiting strong zero-shot performance. We evaluate TOTEM extensively over nearly 500 experiments on three commonly-studied time series tasks with real-world data: imputation (17 baselines, 12 datasets), anomaly detection (19 baselines, 25 datasets), and forecasting (14 baselines, 12 datasets). We conclude that TOTEM matches or outperforms existing state-of-the-art models in both the canonical specialist setting (i.e., training one model on one domain) as well as the generalist setting (i.e., training a single model on many domains), which demonstrates the efficacy of tokenization for general time series analysis. The open-source implementation is available here: https://github.com/SaberaTalukder/TOTEM; a video summary is available here: https://www.youtube.com/watch?v=OqrCpdb6MJk.

==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/ablations/0shot_forecasting_ablation.tex <==
\begin{table}[]
\centering
\caption{Zero Shot Forecasting}
  \vskip -0.0in
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.85} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|cc|cc}
        \toprule
        
        \multicolumn{2}{c}{Models} & 
        \multicolumn{2}{|c}{\rotatebox{0}{\scalebox{0.8}{TOTEM}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeTOTEM}}} \\
    
        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} \\
    
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Neuro2}}}
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{1.138} & \scalebox{0.78}{0.777}
        & \first{\scalebox{0.78}{1.127}} & \first{\scalebox{0.78}{0.773}} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{1.149}} & \first{\scalebox{0.78}{0.785}}
        & \scalebox{0.78}{1.169} & \scalebox{0.78}{0.793} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{1.092}} & \first{\scalebox{0.78}{0.770}}
        & \scalebox{0.78}{1.115} & \scalebox{0.78}{0.780} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{1.045}} & \first{\scalebox{0.78}{0.754}}
        & \scalebox{0.78}{1.070} & \scalebox{0.78}{0.766} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Neuro5}}}
        
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{0.483} & \scalebox{0.78}{0.484}
        & \first{\scalebox{0.78}{0.481}} & \first{\scalebox{0.78}{0.483}} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.495}} & \first{\scalebox{0.78}{0.491}}
        & \scalebox{0.78}{0.508} & \scalebox{0.78}{0.500} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.468}} & \first{\scalebox{0.78}{0.483}}
        & \scalebox{0.78}{0.481} & \scalebox{0.78}{0.491} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.451}} & \first{\scalebox{0.78}{0.477}}
        & \scalebox{0.78}{0.467} & \scalebox{0.78}{0.488} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{River}}}
        
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{1.120} & \scalebox{0.78}{0.582}
        & \first{\scalebox{0.78}{1.102}} & \first{\scalebox{0.78}{0.578}} \\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{1.242} & \scalebox{0.78}{0.635}
        & \first{\scalebox{0.78}{1.207}} & \first{\scalebox{0.78}{0.628}} \\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{1.237} & \scalebox{0.78}{0.626}
        & \first{\scalebox{0.78}{1.190}} & \first{\scalebox{0.78}{0.613}} \\
        
        & \scalebox{0.78}{720}
        & \scalebox{0.78}{1.182} & \scalebox{0.78}{0.604}
        & \first{\scalebox{0.78}{1.149}} & \first{\scalebox{0.78}{0.596}} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Births}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.805}} & \first{\scalebox{0.78}{0.739}}
        & \scalebox{0.78}{0.825} & \scalebox{0.78}{0.751} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.836}} & \first{\scalebox{0.78}{0.752}}
        & \scalebox{0.78}{0.847} & \scalebox{0.78}{0.761} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.809}} & \first{\scalebox{0.78}{0.748}}
        & \scalebox{0.78}{0.831} & \scalebox{0.78}{0.764} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.896}} & \first{\scalebox{0.78}{0.794}}
        & \scalebox{0.78}{0.928} & \scalebox{0.78}{0.813} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Sun}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.446}} & \scalebox{0.78}{0.482}
        & \first{\scalebox{0.78}{0.446}} & \first{\scalebox{0.78}{0.481}} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.462}} & \first{\scalebox{0.78}{0.491}}
        & \scalebox{0.78}{0.478} & \scalebox{0.78}{0.499} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.521}} & \first{\scalebox{0.78}{0.525}}
        & \scalebox{0.78}{0.535} & \scalebox{0.78}{0.532} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.717}} & \first{\scalebox{0.78}{0.625}}
        & \scalebox{0.78}{0.736} & \scalebox{0.78}{0.631} \\
        
        \toprule
        
        \multicolumn{2}{c|}{\scalebox{0.78}{Avg Wins}} &
        \multicolumn{2}{c|}{\first{0.675}} &
        \multicolumn{2}{c}{0.350} \\
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/ablations/dg_0s_forecasting_timetotem_means_stds_ablation.tex <==
\begin{table}[!ht]
\vspace{-10pt}
\centering
\caption{\textbf{TimeTOTEM Ablation - Generalist and Zero-Shot Forecasting}}
  % \vskip -0.0in
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.1} 
  \centering
  \resizebox{0.75\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|c|c}
        \toprule
        
        \multicolumn{2}{c|}{} & \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Mean $\pm$ Std}}} \\
        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} \\
    
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{W}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.173 \pm 0.0012$} & \scalebox{0.78}{$0.218 \pm 0.0006$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.218 \pm 0.0006$} & \scalebox{0.78}{$0.261 \pm 0.0006$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.267 \pm 0.0006$} & \scalebox{0.78}{$0.299 \pm 0.0006$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.337 \pm 0.0010$} & \scalebox{0.78}{$0.347 \pm 0.0006$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{E}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.183 \pm 0.0012$} & \scalebox{0.78}{$0.267 \pm 0.0012$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.189 \pm 0.0006$} & \scalebox{0.78}{$0.275 \pm 0.0000$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.204 \pm 0.0010$} & \scalebox{0.78}{$0.291 \pm 0.0010$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.242 \pm 0.0006$} & \scalebox{0.78}{$0.325 \pm 0.0006$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{T}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.517 \pm 0.0000$} & \scalebox{0.78}{$0.293 \pm 0.0029$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.526 \pm 0.0030$} & \scalebox{0.78}{$0.296 \pm 0.0006$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.552 \pm 0.0015$} & \scalebox{0.78}{$0.304 \pm 0.0015$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.602 \pm 0.0046$} & \scalebox{0.78}{$0.326 \pm 0.0015$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m1}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.428 \pm 0.0090$} & \scalebox{0.78}{$0.420 \pm 0.0040$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.438 \pm 0.0015$} & \scalebox{0.78}{$0.427 \pm 0.0010$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.469 \pm 0.0062$} & \scalebox{0.78}{$0.447 \pm 0.0042$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.546 \pm 0.0081$} & \scalebox{0.78}{$0.493 \pm 0.0017$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m2}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.207 \pm 0.0015$} & \scalebox{0.78}{$0.286 \pm 0.0020$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.269 \pm 0.0015$} & \scalebox{0.78}{$0.325 \pm 0.0010$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.358 \pm 0.0199$} & \scalebox{0.78}{$0.377 \pm 0.0091$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.521 \pm 0.0165$} & \scalebox{0.78}{$0.482 \pm 0.0026$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h1}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.401 \pm 0.0006$} & \scalebox{0.78}{$0.410 \pm 0.0006$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.453 \pm 0.0010$} & \scalebox{0.78}{$0.441 \pm 0.0010$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.496 \pm 0.0017$} & \scalebox{0.78}{$0.468 \pm 0.0006$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.518 \pm 0.0020$} & \scalebox{0.78}{$0.510 \pm 0.0017$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h2}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.305 \pm 0.0006$} & \scalebox{0.78}{$0.346 \pm 0.0006$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.396 \pm 0.0015$} & \scalebox{0.78}{$0.402 \pm 0.0001$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.492 \pm 0.0310$} & \scalebox{0.78}{$0.458 \pm 0.0131$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.599 \pm 0.0105$} & \scalebox{0.78}{$0.531 \pm 0.0026$} \\
        
        \toprule
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{N2}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$1.127 \pm 0.0017$} & \scalebox{0.78}{$0.773 \pm 0.0006$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$1.169 \pm 0.0032$} & \scalebox{0.78}{$0.793 \pm 0.0010$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$1.115 \pm 0.0010$} & \scalebox{0.78}{$0.780 \pm 0.0006$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$1.070 \pm 0.0035$} & \scalebox{0.78}{$0.766 \pm 0.0010$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{N5}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.481 \pm 0.0015$} & \scalebox{0.78}{$0.483 \pm 0.0006$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.508 \pm 0.0012$} & \scalebox{0.78}{$0.500 \pm 0.0000$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.481 \pm 0.0006$} & \scalebox{0.78}{$0.491 \pm 0.0006$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.467 \pm 0.0010$} & \scalebox{0.78}{$0.488 \pm 0.0010$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{R}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$1.102 \pm 0.0031$} & \scalebox{0.78}{$0.578 \pm 0.0021$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$1.207 \pm 0.0036$} & \scalebox{0.78}{$0.628 \pm 0.0017$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$1.190 \pm 0.0021$} & \scalebox{0.78}{$0.613 \pm 0.0010$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$1.149 \pm 0.0017$} & \scalebox{0.78}{$0.596 \pm 0.0020$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{B}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.825 \pm 0.0079$} & \scalebox{0.78}{$0.751 \pm 0.0076$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.847 \pm 0.0021$} & \scalebox{0.78}{$0.761 \pm 0.0012$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.831 \pm 0.0066$} & \scalebox{0.78}{$0.764 \pm 0.0042$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.928 \pm 0.0131$} & \scalebox{0.78}{$0.813 \pm 0.0050$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{S}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.446 \pm 0.0015$} & \scalebox{0.78}{$0.481 \pm 0.0010$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.478 \pm 0.0015$} & \scalebox{0.78}{$0.499 \pm 0.0000$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.535 \pm 0.0012$} & \scalebox{0.78}{$0.532 \pm 0.0006$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.736 \pm 0.0025$} & \scalebox{0.78}{$0.631 \pm 0.0006$} \\

        \toprule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    }
    \label{table:dg_0s_forecasting_timetotem_means_stds_ablation}
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/ablations/dg_and_0shot_forecasting_ablation.tex <==
\begin{table}[ht]
\centering
\caption{Generalist Tokens vs. Time.}
  % \vskip -0.0in
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.1} 
  \centering
  \resizebox{1\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}[b]{c c|cc|cc}
        
        \multicolumn{6}{c}{A. In Domain Performance} \\
        \toprule
        
        \multicolumn{2}{c}{Models} & 
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TOTEM}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeTOTEM}}} \\
    
        \multicolumn{2}{c}{Metric}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} \\
    
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{W}}}
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.172}} & \first{\scalebox{0.78}{0.216}}
        & \scalebox{0.78}{0.173} & \scalebox{0.78}{0.218} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.217}} & \first{\scalebox{0.78}{0.256}}
        & \scalebox{0.78}{0.218} & \scalebox{0.78}{0.261} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.266}} & \first{\scalebox{0.78}{0.295}}
        & \scalebox{0.78}{0.267} & \scalebox{0.78}{0.299} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.334}} & \first{\scalebox{0.78}{0.342}}
        & \scalebox{0.78}{0.337} & \scalebox{0.78}{0.347} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{E}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.179}} & \first{\scalebox{0.78}{0.264}}
        & \scalebox{0.78}{0.183} & \scalebox{0.78}{0.267} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.181}} & \first{\scalebox{0.78}{0.267}}
        & \scalebox{0.78}{0.189} & \scalebox{0.78}{0.275} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.196}} & \first{\scalebox{0.78}{0.283}}
        & \scalebox{0.78}{0.204} & \scalebox{0.78}{0.291} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.230}} & \first{\scalebox{0.78}{0.314}}
        & \scalebox{0.78}{0.242} & \scalebox{0.78}{0.325} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{T}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.507}} & \first{\scalebox{0.78}{0.284}}
        & \scalebox{0.78}{0.517} & \scalebox{0.78}{0.293} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.511}} & \first{\scalebox{0.78}{0.282}}
        & \scalebox{0.78}{0.526} & \scalebox{0.78}{0.296} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.535}} & \first{\scalebox{0.78}{0.292}}
        & \scalebox{0.78}{0.552} & \scalebox{0.78}{0.304} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.580}} & \first{\scalebox{0.78}{0.309}}
        & \scalebox{0.78}{0.602} & \scalebox{0.78}{0.326} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m1}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.374}} & \first{\scalebox{0.78}{0.384}}
        & \scalebox{0.78}{0.428} & \scalebox{0.78}{0.420} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.400}} & \first{\scalebox{0.78}{0.399}}
        & \scalebox{0.78}{0.438} & \scalebox{0.78}{0.427} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.432}} & \first{\scalebox{0.78}{0.424}}
        & \scalebox{0.78}{0.469} & \scalebox{0.78}{0.447} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.487}} & \first{\scalebox{0.78}{0.460}}
        & \scalebox{0.78}{0.546} & \scalebox{0.78}{0.493} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m2}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.198}} & \first{\scalebox{0.78}{0.275}}
        & \scalebox{0.78}{0.207} & \scalebox{0.78}{0.286} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.266}} & \first{\scalebox{0.78}{0.319}}
        & \scalebox{0.78}{0.269} & \scalebox{0.78}{0.325} \\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.365} & \first{\scalebox{0.78}{0.377}}
        & \first{\scalebox{0.78}{0.358}} & \first{\scalebox{0.78}{0.377}} \\
        
        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.588} & \scalebox{0.78}{0.511}
        & \first{\scalebox{0.78}{0.521}} & \first{\scalebox{0.78}{0.482}} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h1}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.382}} & \first{\scalebox{0.78}{0.404}}
        & \scalebox{0.78}{0.401} & \scalebox{0.78}{0.410} \\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{0.463} & \first{\scalebox{0.78}{0.435}}
        & \first{\scalebox{0.78}{0.453}} & \scalebox{0.78}{0.441} \\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.507} & \first{\scalebox{0.78}{0.463}}
        & \first{\scalebox{0.78}{0.496}} & \scalebox{0.78}{0.468} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.517}} & \first{\scalebox{0.78}{0.500}}
        & \scalebox{0.78}{0.518} & \scalebox{0.78}{0.510} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h2}}}
        
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{0.307} & \first{\scalebox{0.78}{0.345}}
        & \first{\scalebox{0.78}{0.305}} & \scalebox{0.78}{0.346} \\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{0.406} & \scalebox{0.78}{0.403}
        & \first{\scalebox{0.78}{0.396}} & \first{\scalebox{0.78}{0.402}} \\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.505} & \scalebox{0.78}{0.460}
        & \first{\scalebox{0.78}{0.492}} & \first{\scalebox{0.78}{0.458}} \\
        
        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.661} & \scalebox{0.78}{0.557}
        & \first{\scalebox{0.78}{0.599}} & \first{\scalebox{0.78}{0.531}} \\
        
        \toprule
        
        \multicolumn{2}{c}{\scalebox{0.78}{\avgwins}} &
        \multicolumn{2}{c|}{\first{78.6\%}} &
        \multicolumn{2}{c}{23.2\%} \\

        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    
      \hspace{-3pt}

      
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}[b]{c c|cc|cc}

        \multicolumn{6}{c}{B. Zero Shot Performance} \\
        \toprule
        
        \multicolumn{2}{c}{Models} & 
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TOTEM}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeTOTEM}}} \\
    
        \multicolumn{2}{c}{Metric}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} \\
    
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{N2}}}
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{1.138} & \scalebox{0.78}{0.777}
        & \first{\scalebox{0.78}{1.127}} & \first{\scalebox{0.78}{0.773}} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{1.149}} & \first{\scalebox{0.78}{0.785}}
        & \scalebox{0.78}{1.169} & \scalebox{0.78}{0.793} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{1.092}} & \first{\scalebox{0.78}{0.770}}
        & \scalebox{0.78}{1.115} & \scalebox{0.78}{0.780} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{1.045}} & \first{\scalebox{0.78}{0.754}}
        & \scalebox{0.78}{1.070} & \scalebox{0.78}{0.766} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{N5}}}
        
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{0.483} & \scalebox{0.78}{0.484}
        & \first{\scalebox{0.78}{0.481}} & \first{\scalebox{0.78}{0.483}} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.495}} & \first{\scalebox{0.78}{0.491}}
        & \scalebox{0.78}{0.508} & \scalebox{0.78}{0.500} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.468}} & \first{\scalebox{0.78}{0.483}}
        & \scalebox{0.78}{0.481} & \scalebox{0.78}{0.491} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.451}} & \first{\scalebox{0.78}{0.477}}
        & \scalebox{0.78}{0.467} & \scalebox{0.78}{0.488} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{R}}}
        
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{1.120} & \scalebox{0.78}{0.582}
        & \first{\scalebox{0.78}{1.102}} & \first{\scalebox{0.78}{0.578}} \\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{1.242} & \scalebox{0.78}{0.635}
        & \first{\scalebox{0.78}{1.207}} & \first{\scalebox{0.78}{0.628}} \\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{1.237} & \scalebox{0.78}{0.626}
        & \first{\scalebox{0.78}{1.190}} & \first{\scalebox{0.78}{0.613}} \\
        
        & \scalebox{0.78}{720}
        & \scalebox{0.78}{1.182} & \scalebox{0.78}{0.604}
        & \first{\scalebox{0.78}{1.149}} & \first{\scalebox{0.78}{0.596}} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{B}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.805}} & \first{\scalebox{0.78}{0.739}}
        & \scalebox{0.78}{0.825} & \scalebox{0.78}{0.751} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.836}} & \first{\scalebox{0.78}{0.752}}
        & \scalebox{0.78}{0.847} & \scalebox{0.78}{0.761} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.809}} & \first{\scalebox{0.78}{0.748}}
        & \scalebox{0.78}{0.831} & \scalebox{0.78}{0.764} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.896}} & \first{\scalebox{0.78}{0.794}}
        & \scalebox{0.78}{0.928} & \scalebox{0.78}{0.813} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{S}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.446}} & \scalebox{0.78}{0.482}
        & \first{\scalebox{0.78}{0.446}} & \first{\scalebox{0.78}{0.481}} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.462}} & \first{\scalebox{0.78}{0.491}}
        & \scalebox{0.78}{0.478} & \scalebox{0.78}{0.499} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.521}} & \first{\scalebox{0.78}{0.525}}
        & \scalebox{0.78}{0.535} & \scalebox{0.78}{0.532} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.717}} & \first{\scalebox{0.78}{0.625}}
        & \scalebox{0.78}{0.736} & \scalebox{0.78}{0.631} \\
        
        \toprule
        
        \multicolumn{2}{c}{\scalebox{0.78}{\avgwins}} &
        \multicolumn{2}{c|}{\first{67.5\%}} &
        \multicolumn{2}{c}{35.0\%} \\

        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
      \label{tab:generalist_tokens_vs_time}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/ablations/dg_forecasting_ablation.tex <==
\begin{table}[]
\centering
\caption{Domain General Forecasting}
  \vskip -0.0in
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.85} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|cc|cc}
        \toprule
        
        \multicolumn{2}{c}{Models} & 
        \multicolumn{2}{|c}{\rotatebox{0}{\scalebox{0.8}{TOTEM}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeTOTEM}}} \\
    
        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} \\
    
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Weather}}}
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.172}} & \first{\scalebox{0.78}{0.216}}
        & \scalebox{0.78}{0.173} & \scalebox{0.78}{0.218} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.217}} & \first{\scalebox{0.78}{0.256}}
        & \scalebox{0.78}{0.218} & \scalebox{0.78}{0.261} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.266}} & \first{\scalebox{0.78}{0.295}}
        & \scalebox{0.78}{0.267} & \scalebox{0.78}{0.299} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.334}} & \first{\scalebox{0.78}{0.342}}
        & \scalebox{0.78}{0.337} & \scalebox{0.78}{0.347} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Electricity}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.179}} & \first{\scalebox{0.78}{0.264}}
        & \scalebox{0.78}{0.183} & \scalebox{0.78}{0.267} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.181}} & \first{\scalebox{0.78}{0.267}}
        & \scalebox{0.78}{0.189} & \scalebox{0.78}{0.275} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.196}} & \first{\scalebox{0.78}{0.283}}
        & \scalebox{0.78}{0.204} & \scalebox{0.78}{0.291} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.230}} & \first{\scalebox{0.78}{0.314}}
        & \scalebox{0.78}{0.242} & \scalebox{0.78}{0.325} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Traffic}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.507}} & \first{\scalebox{0.78}{0.284}}
        & \scalebox{0.78}{0.517} & \scalebox{0.78}{0.293} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.511}} & \first{\scalebox{0.78}{0.282}}
        & \scalebox{0.78}{0.526} & \scalebox{0.78}{0.296} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.535}} & \first{\scalebox{0.78}{0.292}}
        & \scalebox{0.78}{0.552} & \scalebox{0.78}{0.304} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.580}} & \first{\scalebox{0.78}{0.309}}
        & \scalebox{0.78}{0.602} & \scalebox{0.78}{0.326} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTm1}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.374}} & \first{\scalebox{0.78}{0.384}}
        & \scalebox{0.78}{0.428} & \scalebox{0.78}{0.420} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.400}} & \first{\scalebox{0.78}{0.399}}
        & \scalebox{0.78}{0.438} & \scalebox{0.78}{0.427} \\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.432}} & \first{\scalebox{0.78}{0.424}}
        & \scalebox{0.78}{0.469} & \scalebox{0.78}{0.447} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.487}} & \first{\scalebox{0.78}{0.460}}
        & \scalebox{0.78}{0.546} & \scalebox{0.78}{0.493} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTm2}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.198}} & \first{\scalebox{0.78}{0.275}}
        & \scalebox{0.78}{0.207} & \scalebox{0.78}{0.286} \\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.266}} & \first{\scalebox{0.78}{0.319}}
        & \scalebox{0.78}{0.269} & \scalebox{0.78}{0.325} \\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.365} & \first{\scalebox{0.78}{0.377}}
        & \first{\scalebox{0.78}{0.358}} & \first{\scalebox{0.78}{0.377}} \\
        
        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.588} & \scalebox{0.78}{0.511}
        & \first{\scalebox{0.78}{0.521}} & \first{\scalebox{0.78}{0.482}} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTh1}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.382}} & \first{\scalebox{0.78}{0.404}}
        & \scalebox{0.78}{0.401} & \scalebox{0.78}{0.410} \\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{0.463} & \first{\scalebox{0.78}{0.435}}
        & \first{\scalebox{0.78}{0.453}} & \scalebox{0.78}{0.441} \\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.507} & \first{\scalebox{0.78}{0.463}}
        & \first{\scalebox{0.78}{0.496}} & \scalebox{0.78}{0.468} \\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.517}} & \first{\scalebox{0.78}{0.500}}
        & \scalebox{0.78}{0.518} & \scalebox{0.78}{0.510} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTh2}}}
        
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{0.307} & \first{\scalebox{0.78}{0.345}}
        & \first{\scalebox{0.78}{0.305}} & \scalebox{0.78}{0.346} \\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{0.406} & \scalebox{0.78}{0.403}
        & \first{\scalebox{0.78}{0.396}} & \first{\scalebox{0.78}{0.402}} \\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.505} & \scalebox{0.78}{0.460}
        & \first{\scalebox{0.78}{0.492}} & \first{\scalebox{0.78}{0.458}} \\
        
        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.661} & \scalebox{0.78}{0.557}
        & \first{\scalebox{0.78}{0.599}} & \first{\scalebox{0.78}{0.531}} \\
        
        \toprule
        
        \multicolumn{2}{c|}{\scalebox{0.78}{Avg Wins}} &
        \multicolumn{2}{c|}{\first{0.786}} &
        \multicolumn{2}{c}{0.232} \\
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/ablations/ds_forecasting_ablation.tex <==
\begin{table}[ht]
\centering
\caption{Specialist Tokens vs. Time.}
  \vskip -0.0in
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.1} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|cc|cc}
        \toprule
        
        \multicolumn{2}{c}{Models} & 
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TOTEM}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimeTOTEM}}} \\
    
        \multicolumn{2}{c}{Metric}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} \\
    
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{W}}}
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{0.165} & \first{\scalebox{0.78}{0.208}}
        & \first{\scalebox{0.78}{0.164}} & \scalebox{0.78}{0.209}\\
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.207}} & \first{\scalebox{0.78}{0.250}}
        & \scalebox{0.78}{0.209} & \scalebox{0.78}{0.251}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.257}} & \first{\scalebox{0.78}{0.291}}
        & \scalebox{0.78}{0.261} & \scalebox{0.78}{0.293}\\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.326}} & \first{\scalebox{0.78}{0.340}}
        & \scalebox{0.78}{0.332} & \first{\scalebox{0.78}{0.340}}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{E}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.178}} & \scalebox{0.78}{0.263}
        & \scalebox{0.78}{0.179} & \first{\scalebox{0.78}{0.262}}\\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{0.187} & \scalebox{0.78}{0.272}
        & \first{\scalebox{0.78}{0.185}} & \first{\scalebox{0.78}{0.269}}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.199}} & \first{\scalebox{0.78}{0.285}}
        & \scalebox{0.78}{0.204} & \scalebox{0.78}{0.289}\\
        
        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.236}} & \first{\scalebox{0.78}{0.318}}
        & \scalebox{0.78}{0.244} & \scalebox{0.78}{0.325}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{T}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.523}} & \first{\scalebox{0.78}{0.303}}
        & \scalebox{0.78}{0.528} & \scalebox{0.78}{0.310}\\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{0.530} & \first{\scalebox{0.78}{0.303}}
        & \first{\scalebox{0.78}{0.500}} & \scalebox{0.78}{0.349}\\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.549} & \first{\scalebox{0.78}{0.311}}
        & \first{\scalebox{0.78}{0.531}} & \scalebox{0.78}{0.365}\\
        
        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.598} & \first{\scalebox{0.78}{0.331}}
        & \first{\scalebox{0.78}{0.578}} & \scalebox{0.78}{0.398}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m1}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.320}} & \first{\scalebox{0.78}{0.347}}
        & \scalebox{0.78}{0.326} & \scalebox{0.78}{0.355}\\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{0.379} & \first{\scalebox{0.78}{0.382}}
        & \first{\scalebox{0.78}{0.377}} & \scalebox{0.78}{0.386}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.406}} & \first{\scalebox{0.78}{0.402}}
        & \scalebox{0.78}{0.409} & \scalebox{0.78}{0.409}\\
        
        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.471} & \first{\scalebox{0.78}{0.438}}
        & \first{\scalebox{0.78}{0.469}} & \scalebox{0.78}{0.441}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m2}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.176}} & \first{\scalebox{0.78}{0.253}}
        & \first{\scalebox{0.78}{0.176}} & \scalebox{0.78}{0.254}\\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.247}} & \first{\scalebox{0.78}{0.302}}
        & \first{\scalebox{0.78}{0.247}} & \scalebox{0.78}{0.303}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.317}} & \first{\scalebox{0.78}{0.348}}
        & \scalebox{0.78}{0.318} & \scalebox{0.78}{0.350}\\
        
        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.426} & \first{\scalebox{0.78}{0.410}}
        & \first{\scalebox{0.78}{0.419}} & \scalebox{0.78}{0.411}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h1}}}
        
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{0.380} & \first{\scalebox{0.78}{0.394}}
        & \first{\scalebox{0.78}{0.377}} & \scalebox{0.78}{0.395}\\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{0.434} & \first{\scalebox{0.78}{0.427}}
        & \first{\scalebox{0.78}{0.428}} & \scalebox{0.78}{0.428}\\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.490} & \first{\scalebox{0.78}{0.459}}
        & \first{\scalebox{0.78}{0.480}} & \scalebox{0.78}{0.462}\\
        
        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.539} & \first{\scalebox{0.78}{0.513}}
        & \first{\scalebox{0.78}{0.530}} & \scalebox{0.78}{0.522}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h2}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.293}} & \first{\scalebox{0.78}{0.338}}
        & \scalebox{0.78}{0.294} & \first{\scalebox{0.78}{0.338}}\\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{0.375} & \scalebox{0.78}{0.390}
        & \first{\scalebox{0.78}{0.373}} & \first{\scalebox{0.78}{0.389}}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.422}} & \first{\scalebox{0.78}{0.431}}
        & \scalebox{0.78}{0.423} & \scalebox{0.78}{0.433}\\
        
        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.610} & \scalebox{0.78}{0.567}
        & \first{\scalebox{0.78}{0.591}} & \first{\scalebox{0.78}{0.556}}\\
        
        \toprule
        
        \multicolumn{2}{c}{\scalebox{0.78}{\avgwins}} &
        \multicolumn{2}{c|}{\first{67.9\%}} &
        \multicolumn{2}{c}{39.3\%} \\
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
      \label{tab:specialist_tokens_vs_time}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/anomaly_detection/0shot_anomaly_detection.tex <==
\begin{table}[t]
\centering
\caption{Zero Shot Anomaly Detection}
  \vskip -0.0in
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.2} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|c|c}
        \toprule
        
        \multicolumn{2}{c}{Models} & 
        \multicolumn{1}{|c}{\rotatebox{0}{\scalebox{0.8}{\textbf{TOTEM}}}} &
        \multicolumn{1}{c}{\rotatebox{0}{\scalebox{0.8}{GPT2}}} \\
    
    
        \toprule
        
        \multirow{5}{*}{\rotatebox{90}{\scalebox{0.9}{F1 (\%)}}}
        
        & \scalebox{0.78}{Neuro2}
        & \first{\scalebox{0.78}{51.29}}
        & \scalebox{0.78}{39.02}\\
        
        & \scalebox{0.78}{Neuro5}
        & \first{\scalebox{0.78}{51.28}}
        & \scalebox{0.78}{42.19}\\

        & \scalebox{0.78}{River}
        & \first{\scalebox{0.78}{49.39}}
        & \scalebox{0.78}{36.14}\\

        & \scalebox{0.78}{Births}
        & \first{\scalebox{0.78}{49.15}}
        & \scalebox{0.78}{20.81}\\

        & \scalebox{0.78}{Sun}
        & \first{\scalebox{0.78}{52.17}}
        & \scalebox{0.78}{38.12}\\

        \toprule
        
        \multirow{5}{*}{\rotatebox{90}{\scalebox{0.9}{R (\%)}}}
        
        & \scalebox{0.78}{Neuro2}
        & \first{\scalebox{0.78}{76.88}}
        & \scalebox{0.78}{33.69}\\
        
        & \scalebox{0.78}{Neuro5}
        & \first{\scalebox{0.78}{76.84}}
        & \scalebox{0.78}{36.77}\\

        & \scalebox{0.78}{River}
        & \first{\scalebox{0.78}{70.49}}
        & \scalebox{0.78}{29.66}\\

        & \scalebox{0.78}{Births}
        & \first{\scalebox{0.78}{73.71}}
        & \scalebox{0.78}{17.67}\\

        & \scalebox{0.78}{Sun}
        & \first{\scalebox{0.78}{77.36}}
        & \scalebox{0.78}{31.83}\\

        \toprule
        
        \multirow{5}{*}{\rotatebox{90}{\scalebox{0.9}{P (\%)}}}
        
        & \scalebox{0.78}{Neuro2}
        & \scalebox{0.78}{38.49}
        & \first{\scalebox{0.78}{46.43}}\\
        
        & \scalebox{0.78}{Neuro5}
        & \scalebox{0.78}{38.48}
        & \first{\scalebox{0.78}{49.58}}\\

        & \scalebox{0.78}{River}
        & \scalebox{0.78}{38.02}
        & \first{\scalebox{0.78}{46.30}}\\

        & \scalebox{0.78}{Births}
        & \first{\scalebox{0.78}{36.86}}
        & \scalebox{0.78}{25.33}\\

        & \scalebox{0.78}{Sun}
        & \scalebox{0.78}{39.35}
        & \first{\scalebox{0.78}{47.72}}\\

        \toprule

        \multicolumn{2}{c|}{\scalebox{0.78}{Avg Wins}} &
        \multicolumn{1}{c|}{\first{0.733}} &
        \multicolumn{1}{c}{0.267} \\
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/anomaly_detection/dg_0s_anomaly_detection_gpt2_means_stds.tex <==
\begin{table}[!ht]
\centering
\caption{\textbf{GPT2 - Generalist Anomaly Detection $(\uparrow)$}}
\setlength{\tabcolsep}{1pt}
    \begin{tabular}{c c|c}
    \toprule
    
    \multicolumn{2}{c|}{} & 
    \multicolumn{1}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{Mean $\pm$ Std}}}} \\
    
    \toprule
    
    \multirow{10}{*}{\rotatebox{90}{\scalebox{0.9}{\F1}}}
    
    & \scalebox{0.78}{SMD}
    & \scalebox{0.78}{$0.7973 \pm 0.0326$} \\
    
    & \scalebox{0.78}{MSL}
    & \scalebox{0.78}{$0.8017 \pm 0.0205$} \\
    
    & \scalebox{0.78}{SMAP}
    & \scalebox{0.78}{$0.6705 \pm 0.0041$} \\
    
    & \scalebox{0.78}{SWAT}
    & \scalebox{0.78}{$0.8962 \pm 0.0016$} \\
    
    & \scalebox{0.78}{PSM}
    & \scalebox{0.78}{$0.9047 \pm 0.0759$} \\

    & \scalebox{0.78}{N2}
    & \scalebox{0.78}{$0.3902 \pm 0.0596$} \\

    & \scalebox{0.78}{N5}
    & \scalebox{0.78}{$0.4219 \pm 0.0047$} \\

    & \scalebox{0.78}{R}
    & \scalebox{0.78}{$0.3614 \pm 0.0204$} \\

    & \scalebox{0.78}{B}
    & \scalebox{0.78}{$0.2081 \pm 0.0462$} \\

    & \scalebox{0.78}{S}
    & \scalebox{0.78}{$0.3812 \pm 0.0621$} \\
    
    \toprule
    
    \multirow{10}{*}{\rotatebox{90}{\scalebox{0.9}{\Rec}}}
    
    & \scalebox{0.78}{SMD}
    & \scalebox{0.78}{$0.7342 \pm 0.0559$} \\
    
    & \scalebox{0.78}{MSL}
    & \scalebox{0.78}{$0.7848 \pm 0.0277$} \\
    
    & \scalebox{0.78}{SMAP}
    & \scalebox{0.78}{$0.5342 \pm 0.0051$} \\
    
    & \scalebox{0.78}{SWAT}
    & \scalebox{0.78}{$0.8753 \pm 0.0033$} \\
    
    & \scalebox{0.78}{PSM}
    & \scalebox{0.78}{$0.8776 \pm 0.0624$} \\

    & \scalebox{0.78}{N2}
    & \scalebox{0.78}{$0.3369 \pm 0.0592$} \\

    & \scalebox{0.78}{N5}
    & \scalebox{0.78}{$0.3677 \pm 0.0498$} \\

    & \scalebox{0.78}{R}
    & \scalebox{0.78}{$0.2966 \pm 0.0218$} \\

    & \scalebox{0.78}{B}
    & \scalebox{0.78}{$0.1767 \pm 0.0426$} \\

    & \scalebox{0.78}{S}
    & \scalebox{0.78}{$0.3183 \pm 0.0648$} \\
    
    \toprule
    
    \multirow{10}{*}{\rotatebox{90}{\scalebox{0.9}{\Pre}}}
    
    & \scalebox{0.78}{SMD}
    & \scalebox{0.78}{$0.8744 \pm 0.0029$} \\
    
    & \scalebox{0.78}{MSL}
    & \scalebox{0.78}{$0.8195 \pm 0.0130$} \\
    
    & \scalebox{0.78}{SMAP}
    & \scalebox{0.78}{$0.9001 \pm 0.0007$} \\
    
    & \scalebox{0.78}{SWAT}
    & \scalebox{0.78}{$0.9183 \pm 0.0006$} \\
    
    & \scalebox{0.78}{PSM}
    & \scalebox{0.78}{$0.9339 \pm 0.0925$} \\

    & \scalebox{0.78}{N2}
    & \scalebox{0.78}{$0.4643 \pm 0.0561$} \\

    & \scalebox{0.78}{N5}
    & \scalebox{0.78}{$0.4958 \pm 0.0396$} \\

    & \scalebox{0.78}{R}
    & \scalebox{0.78}{$0.4630 \pm 0.0139$} \\

    & \scalebox{0.78}{B}
    & \scalebox{0.78}{$0.2533 \pm 0.0498$} \\

    & \scalebox{0.78}{S}
    & \scalebox{0.78}{$0.4772 \pm 0.5000$} \\
    
    \bottomrule
    
    \end{tabular}
    \label{tab:dg_0s_anomaly_detection_gpt2_means_stds}
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/anomaly_detection/dg_0s_anomaly_detection_totem_means_stds.tex <==
\begin{table}[!ht]
\vspace{-20pt}
\centering
\caption{\textbf{TOTEM - Generalist Anomaly Detection $(\uparrow)$}}
\setlength{\tabcolsep}{1pt}
\resizebox{0.35\columnwidth}{!}{
    \begin{tabular}{c c|c}
    \toprule
    
    \multicolumn{2}{c|}{} & 
    \multicolumn{1}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{Mean $\pm$ Std}}}} \\
    
    \toprule
    
    \multirow{10}{*}{\rotatebox{90}{\scalebox{0.9}{\F1}}}
    
    & \scalebox{0.78}{SMD}
    & \scalebox{0.78}{$0.7864 \pm 0.0386$} \\
    
    & \scalebox{0.78}{MSL}
    & \scalebox{0.78}{$0.8329 \pm 0.0020$} \\
    
    & \scalebox{0.78}{SMAP}
    & \scalebox{0.78}{$0.9251 \pm 0.0014$} \\
    
    & \scalebox{0.78}{SWAT}
    & \scalebox{0.78}{$0.9437 \pm 0.0005$} \\
    
    & \scalebox{0.78}{PSM}
    & \scalebox{0.78}{$0.9578 \pm 0.0002$} \\

    & \scalebox{0.78}{N2}
    & \scalebox{0.78}{$0.5129 \pm 0.0397$} \\

    & \scalebox{0.78}{N5}
    & \scalebox{0.78}{$0.5128 \pm 0.0390$} \\

    & \scalebox{0.78}{R}
    & \scalebox{0.78}{$0.4939 \pm 0.0625$} \\

    & \scalebox{0.78}{B}
    & \scalebox{0.78}{$0.4915 \pm 0.0229$} \\

    & \scalebox{0.78}{S}
    & \scalebox{0.78}{$0.5217 \pm 0.0418$} \\
    
    \toprule
    
    \multirow{10}{*}{\rotatebox{90}{\scalebox{0.9}{\Rec}}}
    
    & \scalebox{0.78}{SMD}
    & \scalebox{0.78}{$0.7207 \pm 0.0565$} \\
    
    & \scalebox{0.78}{MSL}
    & \scalebox{0.78}{$0.8296 \pm 0.0046$} \\
    
    & \scalebox{0.78}{SMAP}
    & \scalebox{0.78}{$0.9148 \pm 0.0020$} \\
    
    & \scalebox{0.78}{SWAT}
    & \scalebox{0.78}{$0.9613 \pm 0.0010$} \\
    
    & \scalebox{0.78}{PSM}
    & \scalebox{0.78}{$0.9390 \pm 0.0004$} \\

    & \scalebox{0.78}{N2}
    & \scalebox{0.78}{$0.7688 \pm 0.0594$} \\

    & \scalebox{0.78}{N5}
    & \scalebox{0.78}{$0.7684 \pm 0.0582$} \\

    & \scalebox{0.78}{R}
    & \scalebox{0.78}{$0.7049 \pm 0.0825$} \\

    & \scalebox{0.78}{B}
    & \scalebox{0.78}{$0.7371 \pm 0.0340$} \\

    & \scalebox{0.78}{S}
    & \scalebox{0.78}{$0.7736 \pm 0.0581$} \\
    
    \toprule
    
    \multirow{10}{*}{\rotatebox{90}{\scalebox{0.9}{\Pre}}}
    
    & \scalebox{0.78}{SMD}
    & \scalebox{0.78}{$0.8666 \pm 0.0114$} \\
    
    & \scalebox{0.78}{MSL}
    & \scalebox{0.78}{$0.8364 \pm 0.0014$} \\
    
    & \scalebox{0.78}{SMAP}
    & \scalebox{0.78}{$0.9356 \pm 0.0009$} \\
    
    & \scalebox{0.78}{SWAT}
    & \scalebox{0.78}{$0.9268 \pm 0.0001$} \\
    
    & \scalebox{0.78}{PSM}
    & \scalebox{0.78}{$0.9774 \pm 0.0002$} \\

    & \scalebox{0.78}{N2}
    & \scalebox{0.78}{$0.3849 \pm 0.0299$} \\

    & \scalebox{0.78}{N5}
    & \scalebox{0.78}{$0.3848 \pm 0.0294$} \\

    & \scalebox{0.78}{R}
    & \scalebox{0.78}{$0.3802 \pm 0.0502$} \\

    & \scalebox{0.78}{B}
    & \scalebox{0.78}{$0.3686 \pm 0.0172$} \\

    & \scalebox{0.78}{S}
    & \scalebox{0.78}{$0.3935 \pm 0.0325$} \\
    
    \bottomrule
    
    \end{tabular}
    \label{tab:dg_0s_anomaly_detection_totem_means_stds}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/anomaly_detection/dg_anomaly_detection.tex <==
\begin{table}[t]
\centering
\caption{Domain General Anomaly Detection}
  \vskip -0.0in
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.2} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|c|c}
        \toprule
        
        \multicolumn{2}{c}{Models} & 
        \multicolumn{1}{|c}{\rotatebox{0}{\scalebox{0.8}{\textbf{TOTEM}}}} &
        \multicolumn{1}{c}{\rotatebox{0}{\scalebox{0.8}{GPT2}}} \\
    
    
        \toprule
        
        \multirow{5}{*}{\rotatebox{90}{\scalebox{0.9}{F1 (\%)}}}
        
        & \scalebox{0.78}{SMD}
        & \scalebox{0.78}{78.64}
        & \first{\scalebox{0.78}{79.73}}\\
        
        & \scalebox{0.78}{MSL}
        & \first{\scalebox{0.78}{83.29}}
        & \scalebox{0.78}{80.17}\\

        & \scalebox{0.78}{SMAP}
        & \first{\scalebox{0.78}{92.51}}
        & \scalebox{0.78}{67.05}\\

        & \scalebox{0.78}{SWAT}
        & \first{\scalebox{0.78}{94.37}}
        & \scalebox{0.78}{89.62}\\

        & \scalebox{0.78}{PSM}
        & \first{\scalebox{0.78}{95.78}}
        & \scalebox{0.78}{90.47}\\

        \toprule
        
        \multirow{5}{*}{\rotatebox{90}{\scalebox{0.9}{R (\%)}}}
        
        & \scalebox{0.78}{SMD}
        & \scalebox{0.78}{72.07}
        & \first{\scalebox{0.78}{73.42}}\\
        
        & \scalebox{0.78}{MSL}
        & \first{\scalebox{0.78}{82.96}}
        & \scalebox{0.78}{78.48}\\

        & \scalebox{0.78}{SMAP}
        & \first{\scalebox{0.78}{91.48}}
        & \scalebox{0.78}{53.42}\\

        & \scalebox{0.78}{SWAT}
        & \first{\scalebox{0.78}{96.13}}
        & \scalebox{0.78}{87.53}\\

        & \scalebox{0.78}{PSM}
        & \first{\scalebox{0.78}{93.90}}
        & \scalebox{0.78}{87.76}\\

        \toprule
        
        \multirow{5}{*}{\rotatebox{90}{\scalebox{0.9}{P (\%)}}}
        
        & \scalebox{0.78}{SMD}
        & \scalebox{0.78}{86.66}
        & \first{\scalebox{0.78}{87.44}}\\
        
        & \scalebox{0.78}{MSL}
        & \first{\scalebox{0.78}{83.64}}
        & \scalebox{0.78}{81.95}\\

        & \scalebox{0.78}{SMAP}
        & \first{\scalebox{0.78}{93.56}}
        & \scalebox{0.78}{90.01}\\

        & \scalebox{0.78}{SWAT}
        & \first{\scalebox{0.78}{92.68}}
        & \scalebox{0.78}{91.83}\\

        & \scalebox{0.78}{PSM}
        & \first{\scalebox{0.78}{97.74}}
        & \scalebox{0.78}{93.39}\\

        \toprule

        \multicolumn{2}{c|}{\scalebox{0.78}{Avg Wins}} &
        \multicolumn{1}{c|}{\first{0.800}} &
        \multicolumn{1}{c}{0.200} \\
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/forecasting/0s_forecasting.tex <==
\begin{table}[]
\centering
\vskip -0.25in
\caption{Zero Shot Forecasting}
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.5} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|cc|cc}
        \toprule
        
        \multicolumn{2}{c}{Models} & 
        \multicolumn{2}{|c}{\rotatebox{0}{\scalebox{0.8}{\textbf{TOTEM}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{GPT2}}}\\
    
        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}\\
    
        \toprule
        
        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Neuro2}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{1.138}} & \first{\scalebox{0.78}{0.777}}
        & \scalebox{0.78}{1.332} & \scalebox{0.78}{0.830}\\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{1.149}} & \first{\scalebox{0.78}{0.785}}
        & \scalebox{0.78}{1.416} & \scalebox{0.78}{0.863}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{1.092}} & \first{\scalebox{0.78}{0.770}}
        & \scalebox{0.78}{1.358} & \scalebox{0.78}{0.851}\\

        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{1.045}} & \first{\scalebox{0.78}{0.754}}
        & \scalebox{0.78}{1.308} & \scalebox{0.78}{0.840}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Neuro5}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.483}} & \first{\scalebox{0.78}{0.484}}
        & \scalebox{0.78}{0.528} & \scalebox{0.78}{0.499}\\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.495}} & \first{\scalebox{0.78}{0.491}}
        & \scalebox{0.78}{0.578} & \scalebox{0.78}{0.524}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.468}} & \first{\scalebox{0.78}{0.483}}
        & \scalebox{0.78}{0.548} & \scalebox{0.78}{0.515}\\

        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.451}} & \first{\scalebox{0.78}{0.477}}
        & \scalebox{0.78}{0.537} & \scalebox{0.78}{0.511}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{River}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{1.120}} & \first{\scalebox{0.78}{0.582}}
        & \scalebox{0.78}{1.465} & \scalebox{0.78}{0.725}\\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{1.242}} & \first{\scalebox{0.78}{0.635}}
        & \scalebox{0.78}{1.638} & \scalebox{0.78}{0.785}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{1.237}} & \first{\scalebox{0.78}{0.626}}
        & \scalebox{0.78}{1.601} & \scalebox{0.78}{0.769}\\

        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{1.182}} & \first{\scalebox{0.78}{0.604}}
        & \scalebox{0.78}{1.552} & \scalebox{0.78}{0.760}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Births}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.805}} & \first{\scalebox{0.78}{0.739}}
        & \scalebox{0.78}{0.838} & \scalebox{0.78}{0.762}\\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.836}} & \first{\scalebox{0.78}{0.752}}
        & \scalebox{0.78}{0.837} & \first{\scalebox{0.78}{0.752}}\\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.809} & \scalebox{0.78}{0.748}
        & \first{\scalebox{0.78}{0.792}} & \first{\scalebox{0.78}{0.738}}\\

        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.896}} & \first{\scalebox{0.78}{0.794}}
        & \scalebox{0.78}{0.927} & \scalebox{0.78}{0.806}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Sun}}}
        
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{0.446} & \scalebox{0.78}{0.482}
        & \first{\scalebox{0.78}{0.443}} & \first{\scalebox{0.78}{0.478}}\\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.462}} & \first{\scalebox{0.78}{0.491}}
        & \scalebox{0.78}{0.481} & \scalebox{0.78}{0.499}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.521}} & \first{\scalebox{0.78}{0.525}}
        & \scalebox{0.78}{0.541} & \scalebox{0.78}{0.533}\\

        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.717}} & \first{\scalebox{0.78}{0.625}}
        & \scalebox{0.78}{0.773} & \scalebox{0.78}{0.643}\\

        \toprule
        
        \multicolumn{2}{c|}{\scalebox{0.78}{Avg Wins}} &
        \multicolumn{2}{c|}{\first{0.900}} &
        \multicolumn{2}{c}{0.125}\\
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/forecasting/dg_and_0shot_forecasting_gpt2_means_stds.tex <==
\begin{table}[!ht]
\vspace{-20pt}
\centering
\caption{\textbf{GPT2 - Generalist and Zero-Shot Forecasting $(\downarrow)$}}
  % \vskip -0.0in
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.1} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|c|c}
        \toprule
        
        \multicolumn{2}{c|}{} & \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Mean $\pm$ Std}}} \\
        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} \\
    
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{W}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.201 \pm 0.0017$} & \scalebox{0.78}{$0.237 \pm 0.0012$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.247 \pm 0.0020$} & \scalebox{0.78}{$0.275 \pm 0.0015$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.298 \pm 0.0006$} & \scalebox{0.78}{$0.311 \pm 0.0006$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.372 \pm 0.0010$} & \scalebox{0.78}{$0.360 \pm 0.0006$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{E}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.194 \pm 0.0012$} & \scalebox{0.78}{$0.278 \pm 0.0021$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.199 \pm 0.0006$} & \scalebox{0.78}{$0.284 \pm 0.0006$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.214 \pm 0.0012$} & \scalebox{0.78}{$0.300 \pm 0.0015$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.255 \pm 0.0006$} & \scalebox{0.78}{$0.331 \pm 0.0012$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{T}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.484 \pm 0.0046$} & \scalebox{0.78}{$0.320 \pm 0.0042$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.488 \pm 0.0006$} & \scalebox{0.78}{$0.320 \pm 0.0006$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.502 \pm 0.0020$} & \scalebox{0.78}{$0.326 \pm 0.0021$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.534 \pm 0.0021$} & \scalebox{0.78}{$0.343 \pm 0.0021$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m1}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.487 \pm 0.0106$} & \scalebox{0.78}{$0.468 \pm 0.0035$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.516 \pm 0.0071$} & \scalebox{0.78}{$0.480 \pm 0.0021$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.548 \pm 0.0015$} & \scalebox{0.78}{$0.499 \pm 0.0015$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.581 \pm 0.0031$} & \scalebox{0.78}{$0.511 \pm 0.0012$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m2}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.243 \pm 0.0021$} & \scalebox{0.78}{$0.315 \pm 0.0021$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.297 \pm 0.0012$} & \scalebox{0.78}{$0.346 \pm 0.0010$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.349 \pm 0.0025$} & \scalebox{0.78}{$0.376 \pm 0.0020$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.439 \pm 0.0010$} & \scalebox{0.78}{$0.423 \pm 0.0010$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h1}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.421 \pm 0.0058$} & \scalebox{0.78}{$0.408 \pm 0.0010$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.480 \pm 0.0026$} & \scalebox{0.78}{$0.436 \pm 0.0020$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.518 \pm 0.0161$} & \scalebox{0.78}{$0.453 \pm 0.0070$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.517 \pm 0.0036$} & \scalebox{0.78}{$0.467 \pm 0.0035$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h2}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.298 \pm 0.0090$} & \scalebox{0.78}{$0.343 \pm 0.0049$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.381 \pm 0.0153$} & \scalebox{0.78}{$0.392 \pm 0.0072$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.406 \pm 0.0271$} & \scalebox{0.78}{$0.419 \pm 0.0144$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.423 \pm 0.0078$} & \scalebox{0.78}{$0.438 \pm 0.0051$} \\
        
        \toprule

        \multicolumn{4}{c}{Zero-Shot} \\
        
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{N2}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$1.332 \pm 0.0012$} & \scalebox{0.78}{$0.830 \pm 0.0010$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$1.416 \pm 0.0080$} & \scalebox{0.78}{$0.863 \pm 0.0025$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$1.358 \pm 0.0123$} & \scalebox{0.78}{$0.851 \pm 0.0042$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$1.308 \pm 0.0026$} & \scalebox{0.78}{$0.840 \pm 0.0010$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{N5}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.528 \pm 0.0006$} & \scalebox{0.78}{$0.499 \pm 0.0010$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.578 \pm 0.0015$} & \scalebox{0.78}{$0.524 \pm 0.0006$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.548 \pm 0.0040$} & \scalebox{0.78}{$0.515 \pm 0.0015$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.537 \pm 0.0006$} & \scalebox{0.78}{$0.511 \pm 0.0006$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{R}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$1.465 \pm 0.0185$} & \scalebox{0.78}{$0.725 \pm 0.0031$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$1.638 \pm 0.0280$} & \scalebox{0.78}{$0.785 \pm 0.0078$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$1.601 \pm 0.0244$} & \scalebox{0.78}{$0.769 \pm 0.0060$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$1.552 \pm 0.0110$} & \scalebox{0.78}{$0.760 \pm 0.0035$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{B}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.838 \pm 0.0149$} & \scalebox{0.78}{$0.762 \pm 0.0071$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.837 \pm 0.0095$} & \scalebox{0.78}{$0.752 \pm 0.0040$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.792 \pm 0.0104$} & \scalebox{0.78}{$0.738 \pm 0.0050$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.927 \pm 0.0066$} & \scalebox{0.78}{$0.806 \pm 0.0038$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{S}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.443 \pm 0.0010$} & \scalebox{0.78}{$0.478 \pm 0.0006$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.481 \pm 0.0006$} & \scalebox{0.78}{$0.499 \pm 0.0006$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.541 \pm 0.0010$} & \scalebox{0.78}{$0.533 \pm 0.0006$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.773 \pm 0.0020$} & \scalebox{0.78}{$0.643 \pm 0.0010$} \\

        \toprule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    }
    \label{table:dg_and_0shot_forecasting_gpt2_means_stds}
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/forecasting/dg_forecasting.tex <==
\begin{table}[]
\centering
\vskip -0.25in
\caption{Generalist Forecasting}
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.7} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|cc|cc}
        \toprule
        
        \multicolumn{2}{c}{Models} & 
        \multicolumn{2}{|c}{\rotatebox{0}{\scalebox{0.8}{\textbf{TOTEM}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{GPT2}}}\\
    
        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}\\
    
        \toprule
        
        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Weather}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.172}} & \first{\scalebox{0.78}{0.216}}
        & \scalebox{0.78}{0.201} & \scalebox{0.78}{0.237}\\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.217}} & \first{\scalebox{0.78}{0.256}}
        & \scalebox{0.78}{0.247} & \scalebox{0.78}{0.275}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.266}} & \first{\scalebox{0.78}{0.295}}
        & \scalebox{0.78}{0.298} & \scalebox{0.78}{0.311}\\

        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.334}} & \first{\scalebox{0.78}{0.342}}
        & \scalebox{0.78}{0.372} & \scalebox{0.78}{0.360}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Electricity}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.179}} & \first{\scalebox{0.78}{0.264}}
        & \scalebox{0.78}{0.194} & \scalebox{0.78}{0.278}\\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.181}} & \first{\scalebox{0.78}{0.267}}
        & \scalebox{0.78}{0.199} & \scalebox{0.78}{0.284}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.196}} & \first{\scalebox{0.78}{0.283}}
        & \scalebox{0.78}{0.214} & \scalebox{0.78}{0.300}\\

        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.230}} & \first{\scalebox{0.78}{0.314}}
        & \scalebox{0.78}{0.255} & \scalebox{0.78}{0.331}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Traffic}}}
        
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{0.507} & \first{\scalebox{0.78}{0.284}}
        & \first{\scalebox{0.78}{0.484}} & \scalebox{0.78}{0.320}\\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{0.511} & \first{\scalebox{0.78}{0.282}}
        & \first{\scalebox{0.78}{0.488}} & \scalebox{0.78}{0.320}\\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.535} & \first{\scalebox{0.78}{0.292}}
        & \first{\scalebox{0.78}{0.502}} & \scalebox{0.78}{0.326}\\

        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.580} & \first{\scalebox{0.78}{0.309}}
        & \first{\scalebox{0.78}{0.534}} & \scalebox{0.78}{0.343}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTm1}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.374}} & \first{\scalebox{0.78}{0.384}}
        & \scalebox{0.78}{0.487} & \scalebox{0.78}{0.468}\\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.400}} & \first{\scalebox{0.78}{0.399}}
        & \scalebox{0.78}{0.516} & \scalebox{0.78}{0.480}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.432}} & \first{\scalebox{0.78}{0.424}}
        & \scalebox{0.78}{0.548} & \scalebox{0.78}{0.499}\\

        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.487}} & \first{\scalebox{0.78}{0.460}}
        & \scalebox{0.78}{0.581} & \scalebox{0.78}{0.511}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTm2}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.198}} & \first{\scalebox{0.78}{0.275}}
        & \scalebox{0.78}{0.243} & \scalebox{0.78}{0.315}\\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.266}} & \first{\scalebox{0.78}{0.319}}
        & \scalebox{0.78}{0.297} & \scalebox{0.78}{0.346}\\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.365} & \scalebox{0.78}{0.377}
        & \first{\scalebox{0.78}{0.349}} & \first{\scalebox{0.78}{0.376}}\\

        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.588} & \scalebox{0.78}{0.511}
        & \first{\scalebox{0.78}{0.439}} & \first{\scalebox{0.78}{0.423}}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTh1}}}
        
        & \scalebox{0.78}{96}
        & \first{\scalebox{0.78}{0.382}} & \first{\scalebox{0.78}{0.404}}
        & \scalebox{0.78}{0.421} & \scalebox{0.78}{0.408}\\
        
        & \scalebox{0.78}{192}
        & \first{\scalebox{0.78}{0.463}} & \first{\scalebox{0.78}{0.435}}
        & \scalebox{0.78}{0.480} & \scalebox{0.78}{0.436}\\
        
        & \scalebox{0.78}{336}
        & \first{\scalebox{0.78}{0.507}} & \scalebox{0.78}{0.463}
        & \scalebox{0.78}{0.518} & \first{\scalebox{0.78}{0.453}}\\

        & \scalebox{0.78}{720}
        & \first{\scalebox{0.78}{0.517}} & \scalebox{0.78}{0.500}
        & \first{\scalebox{0.78}{0.517}} & \first{\scalebox{0.78}{0.467}}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTh2}}}
        
        & \scalebox{0.78}{96}
        & \scalebox{0.78}{0.307} & \scalebox{0.78}{0.345}
        & \first{\scalebox{0.78}{0.298}} & \first{\scalebox{0.78}{0.343}}\\
        
        & \scalebox{0.78}{192}
        & \scalebox{0.78}{0.406} & \scalebox{0.78}{0.403}
        & \first{\scalebox{0.78}{0.381}} & \first{\scalebox{0.78}{0.392}}\\
        
        & \scalebox{0.78}{336}
        & \scalebox{0.78}{0.505} & \scalebox{0.78}{0.460}
        & \first{\scalebox{0.78}{0.406}} & \first{\scalebox{0.78}{0.419}}\\

        & \scalebox{0.78}{720}
        & \scalebox{0.78}{0.661} & \scalebox{0.78}{0.557}
        & \first{\scalebox{0.78}{0.423}} & \first{\scalebox{0.78}{0.438}}\\
        
        \toprule
        
        \multicolumn{2}{c|}{\scalebox{0.78}{Avg Wins}} &
        \multicolumn{2}{c|}{\first{0.679}} &
        \multicolumn{2}{c}{0.339}\\
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/forecasting/ds_forecasting_gpt2_96lookback_mean_stds.tex <==
\begin{table}[!ht]
\vspace{-20pt}
\centering
\caption{\textbf{GPT2 - Specialist Forecasting, Lookback of 96 $(\downarrow)$}}
  % \vskip -0.0in
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.1} 
  \centering
  \resizebox{0.75\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|c|c}
        \toprule
        
        \multicolumn{2}{c|}{} & \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Mean $\pm$ Std}}} \\
        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} \\
    
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{W}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.184 \pm 0.0013$} & \scalebox{0.78}{$0.224 \pm 0.0014$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.231 \pm 0.0012$} & \scalebox{0.78}{$0.263 \pm 0.0009$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.285 \pm 0.0015$} & \scalebox{0.78}{$0.302 \pm 0.0013$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.362 \pm 0.0016$} & \scalebox{0.78}{$0.351 \pm 0.0008$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{E}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.186 \pm 0.0004$} & \scalebox{0.78}{$0.272 \pm 0.0005$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.190 \pm 0.0007$} & \scalebox{0.78}{$0.278 \pm 0.0008$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.204 \pm 0.0003$} & \scalebox{0.78}{$0.291 \pm 0.0005$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.245 \pm 0.0012$} & \scalebox{0.78}{$0.324 \pm 0.0014$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{T}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.471 \pm 0.0016$} & \scalebox{0.78}{$0.311 \pm 0.0016$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.479 \pm 0.0017$} & \scalebox{0.78}{$0.312 \pm 0.0010$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.490 \pm 0.0009$} & \scalebox{0.78}{$0.317 \pm 0.0010$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.524 \pm 0.0019$} & \scalebox{0.78}{$0.336 \pm 0.0018$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m1}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.328 \pm 0.0022$} & \scalebox{0.78}{$0.363 \pm 0.0014$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.368 \pm 0.0006$} & \scalebox{0.78}{$0.382 \pm 0.0004$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.400 \pm 0.0013$} & \scalebox{0.78}{$0.404 \pm 0.0011$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.462 \pm 0.0010$} & \scalebox{0.78}{$0.440 \pm 0.0009$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m2}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.178 \pm 0.0000$} & \scalebox{0.78}{$0.263 \pm 0.0000$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.245 \pm 0.0000$} & \scalebox{0.78}{$0.307 \pm 0.0000$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.307 \pm 0.0000$} & \scalebox{0.78}{$0.346 \pm 0.0000$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.410 \pm 0.0000$} & \scalebox{0.78}{$0.409 \pm 0.0000$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h1}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.379 \pm 0.0032$} & \scalebox{0.78}{$0.397 \pm 0.0007$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.438 \pm 0.0037$} & \scalebox{0.78}{$0.427 \pm 0.0004$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.474 \pm 0.0045$} & \scalebox{0.78}{$0.448 \pm 0.0004$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.496 \pm 0.0066$} & \scalebox{0.78}{$0.475 \pm 0.0033$} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h2}}}
        & \scalebox{0.78}{96} & \scalebox{0.78}{$0.295 \pm 0.0000$} & \scalebox{0.78}{$0.348 \pm 0.0000$} \\
        & \scalebox{0.78}{192} & \scalebox{0.78}{$0.384 \pm 0.0000$} & \scalebox{0.78}{$0.402 \pm 0.0000$} \\
        & \scalebox{0.78}{336} & \scalebox{0.78}{$0.418 \pm 0.0000$} & \scalebox{0.78}{$0.432 \pm 0.0000$} \\
        & \scalebox{0.78}{720} & \scalebox{0.78}{$0.423 \pm 0.0000$} & \scalebox{0.78}{$0.446 \pm 0.0000$} \\
        
        \toprule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    }
    \label{table:ds_forecasting_gpt_96lookback_means_stds}
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/imputation/0shot_imputation.tex <==
\begin{table}[]
\centering
\vskip -0.25in
\caption{Zero Shot Imputation}
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.7} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|cc|cc}
        \toprule
        
        \multicolumn{2}{c}{Models} & 
        \multicolumn{2}{|c}{\rotatebox{0}{\scalebox{0.8}{\textbf{TOTEM}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{GPT2}}}\\
    
        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}\\
    
        \toprule
        
        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Neuro2}}}
        
        & \scalebox{0.78}{12.5\%}
        & \first{\scalebox{0.78}{0.029}} & \first{\scalebox{0.78}{0.120}}
        & \scalebox{0.78}{0.047} & \scalebox{0.78}{0.145}\\
        
        & \scalebox{0.78}{25\%}
        & \first{\scalebox{0.78}{0.033}} & \first{\scalebox{0.78}{0.127}}
        & \scalebox{0.78}{0.064} & \scalebox{0.78}{0.164}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.041}} & \first{\scalebox{0.78}{0.139}}
        & \scalebox{0.78}{0.090} & \scalebox{0.78}{0.191}\\

        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.056}} & \first{\scalebox{0.78}{0.160}}
        & \scalebox{0.78}{0.131} & \scalebox{0.78}{0.228}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Neuro5}}}
        
        & \scalebox{0.78}{12.5\%}
        & \first{\scalebox{0.78}{0.017}} & \first{\scalebox{0.78}{0.085}}
        & \scalebox{0.78}{0.021} & \scalebox{0.78}{0.095}\\
        
        & \scalebox{0.78}{25\%}
        & \first{\scalebox{0.78}{0.019}} & \first{\scalebox{0.78}{0.090}}
        & \scalebox{0.78}{0.028} & \scalebox{0.78}{0.107}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.022}} & \first{\scalebox{0.78}{0.098}}
        & \scalebox{0.78}{0.039} & \scalebox{0.78}{0.123}\\

        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.029}} & \first{\scalebox{0.78}{0.110}}
        & \scalebox{0.78}{0.055} & \scalebox{0.78}{0.145}\\

        \toprule


        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{River}}}
        
        & \scalebox{0.78}{12.5\%}
        & \first{\scalebox{0.78}{0.071}} & \first{\scalebox{0.78}{0.109}}
        & \scalebox{0.78}{0.093} & \scalebox{0.78}{0.119}\\
        
        & \scalebox{0.78}{25\%}
        & \first{\scalebox{0.78}{0.087}} & \first{\scalebox{0.78}{0.117}}
        & \scalebox{0.78}{0.125} & \scalebox{0.78}{0.134}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.112}} & \first{\scalebox{0.78}{0.129}}
        & \scalebox{0.78}{0.167} & \scalebox{0.78}{0.154}\\

        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.148}} & \first{\scalebox{0.78}{0.147}}
        & \scalebox{0.78}{0.220} & \scalebox{0.78}{0.182}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Births}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{0.632} & \scalebox{0.78}{0.642}
        & \first{\scalebox{0.78}{0.392}} & \first{\scalebox{0.78}{0.496}}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{0.693} & \scalebox{0.78}{0.665}
        & \first{\scalebox{0.78}{0.444}} & \first{\scalebox{0.78}{0.523}}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{0.761} & \scalebox{0.78}{0.692}
        & \first{\scalebox{0.78}{0.498}} & \first{\scalebox{0.78}{0.553}}\\

        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{0.827} & \scalebox{0.78}{0.718}
        & \first{\scalebox{0.78}{0.591}} & \first{\scalebox{0.78}{0.599}}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Sun}}}
        
        & \scalebox{0.78}{12.5\%}
        & \first{\scalebox{0.78}{0.057}} & \first{\scalebox{0.78}{0.160}}
        & \scalebox{0.78}{0.070} & \scalebox{0.78}{0.173}\\
        
        & \scalebox{0.78}{25\%}
        & \first{\scalebox{0.78}{0.061}} & \first{\scalebox{0.78}{0.168}}
        & \scalebox{0.78}{0.084} & \scalebox{0.78}{0.189}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.069}} & \first{\scalebox{0.78}{0.178}}
        & \scalebox{0.78}{0.103} & \scalebox{0.78}{0.209}\\

        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.082}} & \first{\scalebox{0.78}{0.193}}
        & \scalebox{0.78}{0.128} & \scalebox{0.78}{0.234}\\
        
        \toprule
        
        \multicolumn{2}{c|}{\scalebox{0.78}{Avg Wins}} &
        \multicolumn{2}{c|}{\first{0.800}} &
        \multicolumn{2}{c}{0.200}\\
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/imputation/dg_and_0s_imputation_totem_means_stds.tex <==
\begin{table}[!ht]
% \centering
\vspace{-20pt}
\caption{\textbf{TOTEM - Generalist Imputation $(\downarrow)$}}
  % \vskip -0.0in
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.1} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|cc}
        \toprule

        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} \\
    
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{W}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.029 \pm 0.0012$} & \scalebox{0.78}{$0.060 \pm 0.0047$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.030 \pm 0.0006$} & \scalebox{0.78}{$0.060 \pm 0.0047$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.032 \pm 0.0006$} & \scalebox{0.78}{$0.062 \pm 0.0030$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.036 \pm 0.0006$} & \scalebox{0.78}{$0.067 \pm 0.0036$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{E}}}
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.065 \pm 0.0020$} & \scalebox{0.78}{$0.171 \pm 0.0032$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.071 \pm 0.0015$} & \scalebox{0.78}{$0.179 \pm 0.0031$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.080 \pm 0.0025$} & \scalebox{0.78}{$0.189 \pm 0.0032$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.095 \pm 0.0026$} & \scalebox{0.78}{$0.205 \pm 0.0032$}\\
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m1}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.041 \pm 0.0006$} & \scalebox{0.78}{$0.132 \pm 0.0015$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.044 \pm 0.0000$} & \scalebox{0.78}{$0.135 \pm 0.0010$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.048 \pm 0.0006$} & \scalebox{0.78}{$0.139 \pm 0.0040$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.058 \pm 0.0010$} & \scalebox{0.78}{$0.152 \pm 0.0000$}\\
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m2}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.040 \pm 0.0020$} & \scalebox{0.78}{$0.125 \pm 0.0067$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.041 \pm 0.0015$} & \scalebox{0.78}{$0.126 \pm 0.0058$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.043 \pm 0.0015$} & \scalebox{0.78}{$0.129 \pm 0.0049$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.048 \pm 0.0010$} & \scalebox{0.78}{$0.136 \pm 0.0038$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h1}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.100 \pm 0.0049$} & \scalebox{0.78}{$0.201 \pm 0.0049$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.108 \pm 0.0049$} & \scalebox{0.78}{$0.209 \pm 0.0038$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.122 \pm 0.0064$} & \scalebox{0.78}{$0.220 \pm 0.0044$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.144 \pm 0.0078$} & \scalebox{0.78}{$0.237 \pm 0.0049$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h2}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.075 \pm 0.0012$} & \scalebox{0.78}{$0.175 \pm 0.0053$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.076 \pm 0.0006$} & \scalebox{0.78}{$0.177 \pm 0.0036$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.093 \pm 0.0222$} & \scalebox{0.78}{$0.195 \pm 0.0200$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.089 \pm 0.0010$} & \scalebox{0.78}{$0.192 \pm 0.0035$}\\

        \toprule

        \multicolumn{4}{c}{Zero-Shot} \\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{N2}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.029 \pm 0.0015$} & \scalebox{0.78}{$0.120 \pm 0.0045$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.033 \pm 0.0010$} & \scalebox{0.78}{$0.127 \pm 0.0035$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.041 \pm 0.0006$} & \scalebox{0.78}{$0.139 \pm 0.0025$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.056 \pm 0.0006$} & \scalebox{0.78}{$0.160 \pm 0.0012$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{N5}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.017 \pm 0.0010$} & \scalebox{0.78}{$0.085 \pm 0.0030$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.019 \pm 0.0010$} & \scalebox{0.78}{$0.090 \pm 0.0030$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.022 \pm 0.0006$} & \scalebox{0.78}{$0.098 \pm 0.0025$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.029 \pm 0.0006$} & \scalebox{0.78}{$0.110 \pm 0.0025$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{R}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.071 \pm 0.0070$} & \scalebox{0.78}{$0.109 \pm 0.0040$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.087 \pm 0.0064$} & \scalebox{0.78}{$0.117 \pm 0.0031$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.112 \pm 0.0050$} & \scalebox{0.78}{$0.129 \pm 0.0035$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.148 \pm 0.0032$} & \scalebox{0.78}{$0.147 \pm 0.0023$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{B}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.632 \pm 0.0087$} & \scalebox{0.78}{$0.642 \pm 0.0068$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.693 \pm 0.0070$} & \scalebox{0.78}{$0.665 \pm 0.0047$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.761 \pm 0.0055$} & \scalebox{0.78}{$0.692 \pm 0.0023$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.827 \pm 0.0044$} & \scalebox{0.78}{$0.718 \pm 0.0000$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{S}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.057 \pm 0.0012$} & \scalebox{0.78}{$0.160 \pm 0.0023$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.061 \pm 0.0006$} & \scalebox{0.78}{$0.168 \pm 0.0021$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.069 \pm 0.0006$} & \scalebox{0.78}{$0.178 \pm 0.0021$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.082 \pm 0.0010$} & \scalebox{0.78}{$0.193 \pm 0.0015$}\\
        
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
      \label{tab:dg_and_0s_imputation_totem_means_stds}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/imputation/dg_and_0shot_imputation_gpt2_means_stds.tex <==
\begin{table}[!ht]
% \centering
\caption{\textbf{GPT2 - Generalist Imputation $(\downarrow)$}}
  % \vskip -0.0in
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.1} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|cc}
        \toprule

        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} \\
    
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{W}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.029 \pm 0.0000$} & \scalebox{0.78}{$0.045 \pm 0.0006$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.033 \pm 0.0006$} & \scalebox{0.78}{$0.048 \pm 0.0006$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.037 \pm 0.0006$} & \scalebox{0.78}{$0.054 \pm 0.0012$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.043 \pm 0.0012$} & \scalebox{0.78}{$0.061 \pm 0.0017$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{E}}}
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.008 \pm 0.0020$} & \scalebox{0.78}{$0.186 \pm 0.0035$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.091 \pm 0.0020$} & \scalebox{0.78}{$0.197 \pm 0.0025$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.108 \pm 0.0021$} & \scalebox{0.78}{$0.213 \pm 0.0026$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.132 \pm 0.0026$} & \scalebox{0.78}{$0.236 \pm 0.0026$}\\
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m1}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.052 \pm 0.0012$} & \scalebox{0.78}{$0.141 \pm 0.0016$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.065 \pm 0.0021$} & \scalebox{0.78}{$0.154 \pm 0.0021$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.085 \pm 0.0038$} & \scalebox{0.78}{$0.171 \pm 0.0026$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.117 \pm 0.0052$} & \scalebox{0.78}{$0.196 \pm 0.0026$}\\
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m2}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.029 \pm 0.0000$} & \scalebox{0.78}{$0.095 \pm 0.0006$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.033 \pm 0.0006$} & \scalebox{0.78}{$0.101 \pm 0.0006$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.038 \pm 0.0006$} & \scalebox{0.78}{$0.110 \pm 0.0012$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.045 \pm 0.0006$} & \scalebox{0.78}{$0.121 \pm 0.0012$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h1}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.113 \pm 0.0012$} & \scalebox{0.78}{$0.217 \pm 0.0021$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.131 \pm 0.0010$} & \scalebox{0.78}{$0.231 \pm 0.0015$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.153 \pm 0.0012$} & \scalebox{0.78}{$0.247 \pm 0.0017$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.182 \pm 0.0006$} & \scalebox{0.78}{$0.266 \pm 0.0012$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h2}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.067 \pm 0.0010$} & \scalebox{0.78}{$0.155 \pm 0.0015$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.071 \pm 0.0006$} & \scalebox{0.78}{$0.160 \pm 0.0015$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.077 \pm 0.0010$} & \scalebox{0.78}{$0.167 \pm 0.0015$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.086 \pm 0.0032$} & \scalebox{0.78}{$0.179 \pm 0.0038$}\\

        \toprule

        \multicolumn{4}{c}{Zero-Shot} \\
        
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{N2}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.047 \pm 0.0006$} & \scalebox{0.78}{$0.145 \pm 0.0015$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.064 \pm 0.0017$} & \scalebox{0.78}{$0.164 \pm 0.0015$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.090 \pm 0.0036$} & \scalebox{0.78}{$0.191 \pm 0.0032$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.131 \pm 0.0051$} & \scalebox{0.78}{$0.228 \pm 0.0044$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{N5}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.021 \pm 0.0006$} & \scalebox{0.78}{$0.095 \pm 0.0012$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.028 \pm 0.0006$} & \scalebox{0.78}{$0.107 \pm 0.0010$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.039 \pm 0.0015$} & \scalebox{0.78}{$0.123 \pm 0.0015$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.055 \pm 0.0015$} & \scalebox{0.78}{$0.145 \pm 0.0023$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{R}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.093 \pm 0.0010$} & \scalebox{0.78}{$0.119 \pm 0.0015$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.125 \pm 0.0006$} & \scalebox{0.78}{$0.134 \pm 0.0026$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.167 \pm 0.0021$} & \scalebox{0.78}{$0.154 \pm 0.0042$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.220 \pm 0.0045$} & \scalebox{0.78}{$0.182 \pm 0.0057$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{B}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.392 \pm 0.0064$} & \scalebox{0.78}{$0.496 \pm 0.0023$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.444 \pm 0.0071$} & \scalebox{0.78}{$0.523 \pm 0.0029$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.498 \pm 0.0080$} & \scalebox{0.78}{$0.553 \pm 0.0023$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.591 \pm 0.0700$} & \scalebox{0.78}{$0.599 \pm 0.0275$}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{s}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{$0.070 \pm 0.0012$} & \scalebox{0.78}{$0.173 \pm 0.0017$}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{$0.084 \pm 0.0010$} & \scalebox{0.78}{$0.189 \pm 0.0015$}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{$0.103 \pm 0.0010$} & \scalebox{0.78}{$0.209 \pm 0.0021$}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{$0.128 \pm 0.0015$} & \scalebox{0.78}{$0.234 \pm 0.0021$}\\
        
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
      \label{tab:dg_and_0shot_imputation_gpt2_means_stds}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/imputation/dg_imputation.tex <==
\begin{table}[]
\centering
\vskip -0.25in
\caption{Domain General Imputation}
  % \vspace{3pt}
  \renewcommand{\arraystretch}{0.7} 
  \centering
  \resizebox{0.5\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|cc|cc}
        \toprule
        
        \multicolumn{2}{c}{Models} & 
        \multicolumn{2}{|c}{\rotatebox{0}{\scalebox{0.8}{\textbf{TOTEM}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{GPT2}}}\\
    
        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}  & \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE}\\
    
        \toprule
        
        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Weather}}}
        
        & \scalebox{0.78}{12.5\%}
        & \first{\scalebox{0.78}{0.029}} & \scalebox{0.78}{0.060}
        & \first{\scalebox{0.78}{0.029}} & \first{\scalebox{0.78}{0.045}}\\
        
        & \scalebox{0.78}{25\%}
        & \first{\scalebox{0.78}{0.030}} & \scalebox{0.78}{0.060}
        & \scalebox{0.78}{0.033} & \first{\scalebox{0.78}{0.048}}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.032}} & \scalebox{0.78}{0.062}
        & \scalebox{0.78}{0.037} & \first{\scalebox{0.78}{0.054}}\\

        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.036}} & \scalebox{0.78}{0.067}
        & \scalebox{0.78}{0.043} & \first{\scalebox{0.78}{0.061}}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{Electricity}}}
        
        & \scalebox{0.78}{12.5\%}
        & \first{\scalebox{0.78}{0.065}} & \first{\scalebox{0.78}{0.171}}
        & \scalebox{0.78}{0.080} & \scalebox{0.78}{0.186}\\
        
        & \scalebox{0.78}{25\%}
        & \first{\scalebox{0.78}{0.071}} & \first{\scalebox{0.78}{0.179}}
        & \scalebox{0.78}{0.091} & \scalebox{0.78}{0.197}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.080}} & \first{\scalebox{0.78}{0.189}}
        & \scalebox{0.78}{0.108} & \scalebox{0.78}{0.213}\\

        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.095}} & \first{\scalebox{0.78}{0.205}}
        & \scalebox{0.78}{0.132} & \scalebox{0.78}{0.236}\\

        \toprule


        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTm1}}}
        
        & \scalebox{0.78}{12.5\%}
        & \first{\scalebox{0.78}{0.041}} & \first{\scalebox{0.78}{0.132}}
        & \scalebox{0.78}{0.052} & \scalebox{0.78}{0.141}\\
        
        & \scalebox{0.78}{25\%}
        & \first{\scalebox{0.78}{0.044}} & \first{\scalebox{0.78}{0.135}}
        & \scalebox{0.78}{0.065} & \scalebox{0.78}{0.154}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.048}} & \first{\scalebox{0.78}{0.139}}
        & \scalebox{0.78}{0.085} & \scalebox{0.78}{0.171}\\

        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.058}} & \first{\scalebox{0.78}{0.152}}
        & \scalebox{0.78}{0.117} & \scalebox{0.78}{0.196}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTm2}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{0.040} & \scalebox{0.78}{0.125}
        & \first{\scalebox{0.78}{0.029}} & \first{\scalebox{0.78}{0.095}}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{0.041} & \scalebox{0.78}{0.126}
        & \first{\scalebox{0.78}{0.033}} & \first{\scalebox{0.78}{0.101}}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{0.043} & \scalebox{0.78}{0.129}
        & \first{\scalebox{0.78}{0.038}} & \first{\scalebox{0.78}{0.110}}\\

        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{0.048} & \scalebox{0.78}{0.136}
        & \first{\scalebox{0.78}{0.045}} & \first{\scalebox{0.78}{0.121}}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTh1}}}
        
        & \scalebox{0.78}{12.5\%}
        & \first{\scalebox{0.78}{0.100}} & \first{\scalebox{0.78}{0.201}}
        & \scalebox{0.78}{0.113} & \scalebox{0.78}{0.217}\\
        
        & \scalebox{0.78}{25\%}
        & \first{\scalebox{0.78}{0.108}} & \first{\scalebox{0.78}{0.209}}
        & \scalebox{0.78}{0.131} & \scalebox{0.78}{0.231}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.122}} & \first{\scalebox{0.78}{0.220}}
        & \scalebox{0.78}{0.153} & \scalebox{0.78}{0.247}\\

        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.144}} & \first{\scalebox{0.78}{0.237}}
        & \scalebox{0.78}{0.182} & \scalebox{0.78}{0.266}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{ETTh2}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{0.075} & \scalebox{0.78}{0.175}
        & \first{\scalebox{0.78}{0.067}} & \first{\scalebox{0.78}{0.155}}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{0.076} & \scalebox{0.78}{0.177}
        & \first{\scalebox{0.78}{0.071}} & \first{\scalebox{0.78}{0.160}}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{0.093} & \scalebox{0.78}{0.195}
        & \first{\scalebox{0.78}{0.077}} & \first{\scalebox{0.78}{0.167}}\\

        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{0.089} & \scalebox{0.78}{0.192}
        & \first{\scalebox{0.78}{0.086}} & \first{\scalebox{0.78}{0.179}}\\
        
        \toprule
        
        \multicolumn{2}{c|}{\scalebox{0.78}{Avg Wins}} &
        \multicolumn{2}{c|}{\first{0.583}} &
        \multicolumn{2}{c}{0.438}\\
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
    }
\end{table}


==> icml_totem_tokenized_time_series_embeddings_for_general_time_series_analysis/tables/imputation/ds_imputation.tex <==
\begin{table*}[t]
% \centering
\caption{\textbf{Specialist Imputation $(\downarrow)$.} Across all datasets, metrics, and masking percentages, TOTEM has the highest \avgwins (\first{52.1\%}), followed by GPT2 (\second{35.4\%}). TOTEM values are means from 3 seeds; baseline values are from \cite{zhou2023one, wu2022timesnet}.}
  % \vskip -0.0in
  % \vspace{-10pt}
  \renewcommand{\arraystretch}{0.1} 
  \centering
  \resizebox{1\columnwidth}{!}{
      \begin{threeparttable}
      \begin{small}
      \renewcommand{\multirowsetup}{\centering}
      
      \setlength{\tabcolsep}{1pt}
      \begin{tabular}{c c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
        \toprule
        
        \multicolumn{2}{c|}{Model} & 
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\multitask{\textbf{TOTEM}}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\multitask{GPT2}}}} &
        \multicolumn{2}{c|}{\rotatebox{0}{\scalebox{0.8}{\multitask{TiNet}}}}  &
        \multicolumn{2}{|c}{\rotatebox{0}{\scalebox{0.8}{\singletask{Patch}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\singletask{ETS}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\singletask{FED}}}}&
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\singletask{Stat}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\singletask{Auto}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\singletask{Inf}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\singletask{Re}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\singletask{LiTS}}}} &
        \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\singletask{Dlin}}}} \\
    
        \multicolumn{2}{c|}{Metric}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae}  & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae} & \scalebox{0.78}{\mse} & \scalebox{0.78}{\mae}\\
    
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{W}}}
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{0.028} & \second{\scalebox{0.78}{0.046}}
        & \second{\scalebox{0.78}{0.026}} & \scalebox{0.78}{0.049}
        & \first{\scalebox{0.78}{0.025}} & \first{\scalebox{0.78}{0.045}}
        & \scalebox{0.78}{0.029} & \scalebox{0.78}{0.049}
        & \scalebox{0.78}{0.057} & \scalebox{0.78}{0.141}
        & \scalebox{0.78}{0.041} & \scalebox{0.78}{0.107}
        & \scalebox{0.78}{0.027} & \scalebox{0.78}{0.051}
        & \second{\scalebox{0.78}{0.026}} & \third{\scalebox{0.78}{0.047}}
        & \scalebox{0.78}{0.037} & \scalebox{0.78}{0.093}
        & \scalebox{0.78}{0.031} & \scalebox{0.78}{0.076}
        & \scalebox{0.78}{0.047} & \scalebox{0.78}{0.101}
        & \scalebox{0.78}{0.039} & \scalebox{0.78}{0.084}\\
        
        & \scalebox{0.78}{25\%}
        & \second{\scalebox{0.78}{0.029}} & \first{\scalebox{0.78}{0.047}}
        & \first{\scalebox{0.78}{0.028}} & \second{\scalebox{0.78}{0.052}}
        & \second{\scalebox{0.78}{0.029}} & \second{\scalebox{0.78}{0.052}}
        & \scalebox{0.78}{0.031} & \scalebox{0.78}{0.053}
        & \scalebox{0.78}{0.065} & \scalebox{0.78}{0.155}
        & \scalebox{0.78}{0.064} & \scalebox{0.78}{0.163}
        & \second{\scalebox{0.78}{0.029}} & \scalebox{0.78}{0.056}
        & \scalebox{0.78}{0.030} & \scalebox{0.78}{0.054}
        & \scalebox{0.78}{0.042} & \scalebox{0.78}{0.100}
        & \scalebox{0.78}{0.035} & \scalebox{0.78}{0.082}
        & \scalebox{0.78}{0.052} & \scalebox{0.78}{0.111}
        & \scalebox{0.78}{0.048} & \scalebox{0.78}{0.103}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.031}} & \first{\scalebox{0.78}{0.048}}
        & \scalebox{0.78}{0.033} & \scalebox{0.78}{0.060}
        & \first{\scalebox{0.78}{0.031}} & \second{\scalebox{0.78}{0.057}}
        & \scalebox{0.78}{0.035} & \third{\scalebox{0.78}{0.058}}
        & \scalebox{0.78}{0.081} & \scalebox{0.78}{0.180}
        & \scalebox{0.78}{0.107} & \scalebox{0.78}{0.229}
        & \scalebox{0.78}{0.033} & \scalebox{0.78}{0.062}
        & \second{\scalebox{0.78}{0.032}} & \scalebox{0.78}{0.060}
        & \scalebox{0.78}{0.049} & \scalebox{0.78}{0.111}
        & \scalebox{0.78}{0.040} & \scalebox{0.78}{0.091}
        & \scalebox{0.78}{0.058} & \scalebox{0.78}{0.121}
        & \scalebox{0.78}{0.057} & \scalebox{0.78}{0.117}\\
        
        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.033}} & \first{\scalebox{0.78}{0.052}}
        & \third{\scalebox{0.78}{0.037}} & \scalebox{0.78}{0.065}
        & \second{\scalebox{0.78}{0.034}} & \second{\scalebox{0.78}{0.062}}
        & \scalebox{0.78}{0.038} & \third{\scalebox{0.78}{0.063}}
        & \scalebox{0.78}{0.102} & \scalebox{0.78}{0.207}
        & \scalebox{0.78}{0.183} & \scalebox{0.78}{0.312}
        & \third{\scalebox{0.78}{0.037}} & \scalebox{0.78}{0.068}
        & \third{\scalebox{0.78}{0.037}} & \scalebox{0.78}{0.067}
        & \scalebox{0.78}{0.053} & \scalebox{0.78}{0.114}
        & \scalebox{0.78}{0.046} & \scalebox{0.78}{0.099}
        & \scalebox{0.78}{0.065} & \scalebox{0.78}{0.133}
        & \scalebox{0.78}{0.066} & \scalebox{0.78}{0.134}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{E}}}
        & \scalebox{0.78}{12.5\%}
        & \first{\scalebox{0.78}{0.054}} & \first{\scalebox{0.78}{0.154}}
        & \third{\scalebox{0.78}{0.080}} & \third{\scalebox{0.78}{0.194}}
        & \scalebox{0.78}{0.085} & \scalebox{0.78}{0.202}
        & \second{\scalebox{0.78}{0.055}} & \second{\scalebox{0.78}{0.160}}
        & \scalebox{0.78}{0.196} & \scalebox{0.78}{0.321}
        & \scalebox{0.78}{0.107} & \scalebox{0.78}{0.237}
        & \scalebox{0.78}{0.093} & \scalebox{0.78}{0.210}
        & \scalebox{0.78}{0.089} & \scalebox{0.78}{0.210}
        & \scalebox{0.78}{0.218} & \scalebox{0.78}{0.326}
        & \scalebox{0.78}{0.190} & \scalebox{0.78}{0.308}
        & \scalebox{0.78}{0.102} & \scalebox{0.78}{0.229}
        & \scalebox{0.78}{0.092} & \scalebox{0.78}{0.214}\\
        
        & \scalebox{0.78}{25\%}
        & \first{\scalebox{0.78}{0.059}} & \first{\scalebox{0.78}{0.160}}
        & \third{\scalebox{0.78}{0.087}} & \third{\scalebox{0.78}{0.203}}
        & \scalebox{0.78}{0.089} & \scalebox{0.78}{0.206}
        & \second{\scalebox{0.78}{0.065}} & \second{\scalebox{0.78}{0.175}}
        & \scalebox{0.78}{0.207} & \scalebox{0.78}{0.332}
        & \scalebox{0.78}{0.120} & \scalebox{0.78}{0.251}
        & \scalebox{0.78}{0.097} & \scalebox{0.78}{0.214}
        & \scalebox{0.78}{0.096} & \scalebox{0.78}{0.220}
        & \scalebox{0.78}{0.219} & \scalebox{0.78}{0.326}
        & \scalebox{0.78}{0.197} & \scalebox{0.78}{0.312}
        & \scalebox{0.78}{0.121} & \scalebox{0.78}{0.252}
        & \scalebox{0.78}{0.118} & \scalebox{0.78}{0.247}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.067}} & \first{\scalebox{0.78}{0.169}}
        & \third{\scalebox{0.78}{0.094}} & \third{\scalebox{0.78}{0.211}}
        & \third{\scalebox{0.78}{0.094}} & \scalebox{0.78}{0.213}
        & \second{\scalebox{0.78}{0.076}} & \second{\scalebox{0.78}{0.189}}
        & \scalebox{0.78}{0.219} & \scalebox{0.78}{0.344}
        & \scalebox{0.78}{0.136} & \scalebox{0.78}{0.266}
        & \scalebox{0.78}{0.102} & \scalebox{0.78}{0.220}
        & \scalebox{0.78}{0.104} & \scalebox{0.78}{0.229}
        & \scalebox{0.78}{0.222} & \scalebox{0.78}{0.328}
        & \scalebox{0.78}{0.203} & \scalebox{0.78}{0.315}
        & \scalebox{0.78}{0.141} & \scalebox{0.78}{0.273}
        & \scalebox{0.78}{0.144} & \scalebox{0.78}{0.276}\\
        
        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.079}} & \first{\scalebox{0.78}{0.183}}
        & \scalebox{0.78}{0.101} & \third{\scalebox{0.78}{0.220}}
        & \third{\scalebox{0.78}{0.100}} & \scalebox{0.78}{0.221}
        & \second{\scalebox{0.78}{0.091}} & \second{\scalebox{0.78}{0.208}}
        & \scalebox{0.78}{0.235} & \scalebox{0.78}{0.357}
        & \scalebox{0.78}{0.158} & \scalebox{0.78}{0.284}
        & \scalebox{0.78}{0.108} & \scalebox{0.78}{0.228}
        & \scalebox{0.78}{0.113} & \scalebox{0.78}{0.239}
        & \scalebox{0.78}{0.228} & \scalebox{0.78}{0.331}
        & \scalebox{0.78}{0.210} & \scalebox{0.78}{0.319}
        & \scalebox{0.78}{0.160} & \scalebox{0.78}{0.293}
        & \scalebox{0.78}{0.175} & \scalebox{0.78}{0.305}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m1}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{0.049} & \scalebox{0.78}{0.125}
        & \first{\scalebox{0.78}{0.017}} & \first{\scalebox{0.78}{0.085}}
        & \second{\scalebox{0.78}{0.019}} & \second{\scalebox{0.78}{0.092}}
        & \scalebox{0.78}{0.041} & \scalebox{0.78}{0.130}
        & \scalebox{0.78}{0.067} & \scalebox{0.78}{0.188}
        & \scalebox{0.78}{0.035} & \scalebox{0.78}{0.135}
        & \third{\scalebox{0.78}{0.026}} & \third{\scalebox{0.78}{0.107}}
        & \scalebox{0.78}{0.034} & \scalebox{0.78}{0.124}
        & \scalebox{0.78}{0.047} & \scalebox{0.78}{0.155}
        & \scalebox{0.78}{0.032} & \scalebox{0.78}{0.126}
        & \scalebox{0.78}{0.075} & \scalebox{0.78}{0.180}
        & \scalebox{0.78}{0.058} & \scalebox{0.78}{0.162}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{0.052} & \scalebox{0.78}{0.128}
        & \first{\scalebox{0.78}{0.022}} & \first{\scalebox{0.78}{0.096}}
        & \second{\scalebox{0.78}{0.023}} & \second{\scalebox{0.78}{0.101}}
        & \scalebox{0.78}{0.044} & \scalebox{0.78}{0.135}
        & \scalebox{0.78}{0.096} & \scalebox{0.78}{0.229}
        & \scalebox{0.78}{0.052} & \scalebox{0.78}{0.166}
        & \third{\scalebox{0.78}{0.032}} & \third{\scalebox{0.78}{0.119}}
        & \scalebox{0.78}{0.046} & \scalebox{0.78}{0.144}
        & \scalebox{0.78}{0.063} & \scalebox{0.78}{0.180}
        & \scalebox{0.78}{0.042} & \scalebox{0.78}{0.146}
        & \scalebox{0.78}{0.093} & \scalebox{0.78}{0.206}
        & \scalebox{0.78}{0.080} & \scalebox{0.78}{0.193}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{0.055} & \scalebox{0.78}{0.132}
        & \first{\scalebox{0.78}{0.029}} & \first{\scalebox{0.78}{0.111}}
        & \first{\scalebox{0.78}{0.029}} & \first{\scalebox{0.78}{0.111}}
        & \scalebox{0.78}{0.049} & \scalebox{0.78}{0.143}
        & \scalebox{0.78}{0.133} & \scalebox{0.78}{0.271}
        & \scalebox{0.78}{0.069} & \scalebox{0.78}{0.191}
        & \third{\scalebox{0.78}{0.039}} & \third{\scalebox{0.78}{0.131}}
        & \scalebox{0.78}{0.057} & \scalebox{0.78}{0.161}
        & \scalebox{0.78}{0.079} & \scalebox{0.78}{0.200}
        & \scalebox{0.78}{0.063} & \scalebox{0.78}{0.182}
        & \scalebox{0.78}{0.113} & \scalebox{0.78}{0.231}
        & \scalebox{0.78}{0.103} & \scalebox{0.78}{0.219}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{0.061} & \third{\scalebox{0.78}{0.139}}
        & \second{\scalebox{0.78}{0.040}} & \second{\scalebox{0.78}{0.128}}
        & \first{\scalebox{0.78}{0.036}} & \first{\scalebox{0.78}{0.124}}
        & \scalebox{0.78}{0.055} & \scalebox{0.78}{0.151}
        & \scalebox{0.78}{0.186} & \scalebox{0.78}{0.323}
        & \scalebox{0.78}{0.089} & \scalebox{0.78}{0.218}
        & \third{\scalebox{0.78}{0.047}} & \scalebox{0.78}{0.145}
        & \scalebox{0.78}{0.067} & \scalebox{0.78}{0.174}
        & \scalebox{0.78}{0.093} & \scalebox{0.78}{0.218}
        & \scalebox{0.78}{0.082} & \scalebox{0.78}{0.208}
        & \scalebox{0.78}{0.134} & \scalebox{0.78}{0.255}
        & \scalebox{0.78}{0.132} & \scalebox{0.78}{0.248}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{m2}}}
        
        & \scalebox{0.78}{12.5\%}
        & \first{\scalebox{0.78}{0.016}} & \second{\scalebox{0.78}{0.078}}
        & \second{\scalebox{0.78}{0.017}} & \first{\scalebox{0.78}{0.076}}
        & \third{\scalebox{0.78}{0.018}} & \third{\scalebox{0.78}{0.080}}
        & \scalebox{0.78}{0.026} & \scalebox{0.78}{0.094}
        & \scalebox{0.78}{0.108} & \scalebox{0.78}{0.239}
        & \scalebox{0.78}{0.056} & \scalebox{0.78}{0.159}
        & \scalebox{0.78}{0.021} & \scalebox{0.78}{0.088}
        & \scalebox{0.78}{0.023} & \scalebox{0.78}{0.092}
        & \scalebox{0.78}{0.133} & \scalebox{0.78}{0.270}
        & \scalebox{0.78}{0.108} & \scalebox{0.78}{0.228}
        & \scalebox{0.78}{0.034} & \scalebox{0.78}{0.127}
        & \scalebox{0.78}{0.062} & \scalebox{0.78}{0.166}\\
        
        & \scalebox{0.78}{25\%}
        & \first{\scalebox{0.78}{0.017}} & \second{\scalebox{0.78}{0.081}}
        & \second{\scalebox{0.78}{0.020}} & \first{\scalebox{0.78}{0.080}}
        & \second{\scalebox{0.78}{0.020}} & \third{\scalebox{0.78}{0.085}}
        & \scalebox{0.78}{0.028} & \scalebox{0.78}{0.099}
        & \scalebox{0.78}{0.164} & \scalebox{0.78}{0.294}
        & \scalebox{0.78}{0.080} & \scalebox{0.78}{0.195}
        & \scalebox{0.78}{0.024} & \scalebox{0.78}{0.096}
        & \scalebox{0.78}{0.026} & \scalebox{0.78}{0.101}
        & \scalebox{0.78}{0.135} & \scalebox{0.78}{0.272}
        & \scalebox{0.78}{0.136} & \scalebox{0.78}{0.262}
        & \scalebox{0.78}{0.042} & \scalebox{0.78}{0.143}
        & \scalebox{0.78}{0.085} & \scalebox{0.78}{0.196}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.018}} & \first{\scalebox{0.78}{0.084}}
        & \second{\scalebox{0.78}{0.022}} & \second{\scalebox{0.78}{0.087}}
        & \third{\scalebox{0.78}{0.023}} & \third{\scalebox{0.78}{0.091}}
        & \scalebox{0.78}{0.030} & \scalebox{0.78}{0.104}
        & \scalebox{0.78}{0.237} & \scalebox{0.78}{0.356}
        & \scalebox{0.78}{0.110} & \scalebox{0.78}{0.231}
        & \scalebox{0.78}{0.027} & \scalebox{0.78}{0.103}
        & \scalebox{0.78}{0.030} & \scalebox{0.78}{0.108}
        & \scalebox{0.78}{0.155} & \scalebox{0.78}{0.293}
        & \scalebox{0.78}{0.175} & \scalebox{0.78}{0.300}
        & \scalebox{0.78}{0.051} & \scalebox{0.78}{0.159}
        & \scalebox{0.78}{0.106} & \scalebox{0.78}{0.222}\\
        
        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.020}} & \first{\scalebox{0.78}{0.088}}
        & \second{\scalebox{0.78}{0.025}} & \second{\scalebox{0.78}{0.095}}
        & \third{\scalebox{0.78}{0.026}} & \third{\scalebox{0.78}{0.098}}
        & \scalebox{0.78}{0.034} & \scalebox{0.78}{0.110}
        & \scalebox{0.78}{0.323} & \scalebox{0.78}{0.421}
        & \scalebox{0.78}{0.156} & \scalebox{0.78}{0.276}
        & \scalebox{0.78}{0.030} & \scalebox{0.78}{0.108}
        & \scalebox{0.78}{0.035} & \scalebox{0.78}{0.119}
        & \scalebox{0.78}{0.200} & \scalebox{0.78}{0.333}
        & \scalebox{0.78}{0.211} & \scalebox{0.78}{0.329}
        & \scalebox{0.78}{0.059} & \scalebox{0.78}{0.174}
        & \scalebox{0.78}{0.131} & \scalebox{0.78}{0.247}\\
        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h1}}}
        
        & \scalebox{0.78}{12.5\%}
        & \scalebox{0.78}{0.119} & \scalebox{0.78}{0.212}
        & \first{\scalebox{0.78}{0.043}} & \first{\scalebox{0.78}{0.140}}
        & \second{\scalebox{0.78}{0.057}} & \second{\scalebox{0.78}{0.159}}
        & \scalebox{0.78}{0.093} & \scalebox{0.78}{0.201}
        & \scalebox{0.78}{0.126} & \scalebox{0.78}{0.263}
        & \scalebox{0.78}{0.070} & \scalebox{0.78}{0.190}
        & \third{\scalebox{0.78}{0.060}} & \third{\scalebox{0.78}{0.165}}
        & \scalebox{0.78}{0.074} & \scalebox{0.78}{0.182}
        & \scalebox{0.78}{0.114} & \scalebox{0.78}{0.234}
        & \scalebox{0.78}{0.074} & \scalebox{0.78}{0.194}
        & \scalebox{0.78}{0.240} & \scalebox{0.78}{0.345}
        & \scalebox{0.78}{0.151} & \scalebox{0.78}{0.267}\\
        
        & \scalebox{0.78}{25\%}
        & \scalebox{0.78}{0.127} & \scalebox{0.78}{0.220}
        & \first{\scalebox{0.78}{0.054}} & \first{\scalebox{0.78}{0.156}}
        & \second{\scalebox{0.78}{0.069}} & \second{\scalebox{0.78}{0.178}}
        & \scalebox{0.78}{0.107} & \scalebox{0.78}{0.217}
        & \scalebox{0.78}{0.169} & \scalebox{0.78}{0.304}
        & \scalebox{0.78}{0.106} & \scalebox{0.78}{0.236}
        & \third{\scalebox{0.78}{0.080}} & \third{\scalebox{0.78}{0.189}}
        & \scalebox{0.78}{0.090} & \scalebox{0.78}{0.203}
        & \scalebox{0.78}{0.140} & \scalebox{0.78}{0.262}
        & \scalebox{0.78}{0.102} & \scalebox{0.78}{0.227}
        & \scalebox{0.78}{0.265} & \scalebox{0.78}{0.364}
        & \scalebox{0.78}{0.180} & \scalebox{0.78}{0.292}\\
        
        & \scalebox{0.78}{37.5\%}
        & \scalebox{0.78}{0.138} & \scalebox{0.78}{0.230}
        & \first{\scalebox{0.78}{0.072}} & \first{\scalebox{0.78}{0.180}}
        & \second{\scalebox{0.78}{0.084}} & \second{\scalebox{0.78}{0.196}}
        & \scalebox{0.78}{0.120} & \scalebox{0.78}{0.230}
        & \scalebox{0.78}{0.220} & \scalebox{0.78}{0.347}
        & \scalebox{0.78}{0.124} & \scalebox{0.78}{0.258}
        & \third{\scalebox{0.78}{0.102}} & \third{\scalebox{0.78}{0.212}}
        & \scalebox{0.78}{0.109} & \scalebox{0.78}{0.222}
        & \scalebox{0.78}{0.174} & \scalebox{0.78}{0.293}
        & \scalebox{0.78}{0.135} & \scalebox{0.78}{0.261}
        & \scalebox{0.78}{0.296} & \scalebox{0.78}{0.382}
        & \scalebox{0.78}{0.215} & \scalebox{0.78}{0.318}\\
        
        & \scalebox{0.78}{50\%}
        & \scalebox{0.78}{0.157} & \scalebox{0.78}{0.247}
        & \second{\scalebox{0.78}{0.107}} & \second{\scalebox{0.78}{0.216}}
        & \first{\scalebox{0.78}{0.102}} & \first{\scalebox{0.78}{0.215}}
        & \scalebox{0.78}{0.141} & \scalebox{0.78}{0.248}
        & \scalebox{0.78}{0.293} & \scalebox{0.78}{0.402}
        & \scalebox{0.78}{0.165} & \scalebox{0.78}{0.299}
        & \third{\scalebox{0.78}{0.133}} & \third{\scalebox{0.78}{0.240}}
        & \scalebox{0.78}{0.137} & \scalebox{0.78}{0.248}
        & \scalebox{0.78}{0.215} & \scalebox{0.78}{0.325}
        & \scalebox{0.78}{0.179} & \scalebox{0.78}{0.298}
        & \scalebox{0.78}{0.334} & \scalebox{0.78}{0.404}
        & \scalebox{0.78}{0.257} & \scalebox{0.78}{0.347}\\

        \toprule

        \multirow{4}{*}{\rotatebox{90}{\scalebox{0.9}{h2}}}
        
        & \scalebox{0.78}{12.5\%}
        & \second{\scalebox{0.78}{0.040}} & \second{\scalebox{0.78}{0.129}}
        & \first{\scalebox{0.78}{0.039}} & \first{\scalebox{0.78}{0.125}}
        & \second{\scalebox{0.78}{0.040}} & \third{\scalebox{0.78}{0.130}}
        & \scalebox{0.78}{0.057} & \scalebox{0.78}{0.152}
        & \scalebox{0.78}{0.187} & \scalebox{0.78}{0.319}
        & \scalebox{0.78}{0.095} & \scalebox{0.78}{0.212}
        & \scalebox{0.78}{0.042} & \scalebox{0.78}{0.133}
        & \scalebox{0.78}{0.044} & \scalebox{0.78}{0.138}
        & \scalebox{0.78}{0.305} & \scalebox{0.78}{0.431}
        & \scalebox{0.78}{0.163} & \scalebox{0.78}{0.289}
        & \scalebox{0.78}{0.101} & \scalebox{0.78}{0.231}
        & \scalebox{0.78}{0.100} & \scalebox{0.78}{0.216}\\
        
        & \scalebox{0.78}{25\%}
        & \first{\scalebox{0.78}{0.041}} & \first{\scalebox{0.78}{0.131}}
        & \second{\scalebox{0.78}{0.044}} & \second{\scalebox{0.78}{0.135}}
        & \third{\scalebox{0.78}{0.046}} & \third{\scalebox{0.78}{0.141}}
        & \scalebox{0.78}{0.061} & \scalebox{0.78}{0.158}
        & \scalebox{0.78}{0.279} & \scalebox{0.78}{0.390}
        & \scalebox{0.78}{0.137} & \scalebox{0.78}{0.258}
        & \scalebox{0.78}{0.049} & \scalebox{0.78}{0.147}
        & \scalebox{0.78}{0.050} & \scalebox{0.78}{0.149}
        & \scalebox{0.78}{0.322} & \scalebox{0.78}{0.444}
        & \scalebox{0.78}{0.206} & \scalebox{0.78}{0.331}
        & \scalebox{0.78}{0.115} & \scalebox{0.78}{0.246}
        & \scalebox{0.78}{0.127} & \scalebox{0.78}{0.247}\\
        
        & \scalebox{0.78}{37.5\%}
        & \first{\scalebox{0.78}{0.043}} & \first{\scalebox{0.78}{0.136}}
        & \second{\scalebox{0.78}{0.051}} & \second{\scalebox{0.78}{0.147}}
        & \third{\scalebox{0.78}{0.052}} & \third{\scalebox{0.78}{0.151}}
        & \scalebox{0.78}{0.067} & \scalebox{0.78}{0.166}
        & \scalebox{0.78}{0.400} & \scalebox{0.78}{0.465}
        & \scalebox{0.78}{0.187} & \scalebox{0.78}{0.304}
        & \scalebox{0.78}{0.056} & \scalebox{0.78}{0.158}
        & \scalebox{0.78}{0.060} & \scalebox{0.78}{0.163}
        & \scalebox{0.78}{0.353} & \scalebox{0.78}{0.462}
        & \scalebox{0.78}{0.252} & \scalebox{0.78}{0.370}
        & \scalebox{0.78}{0.126} & \scalebox{0.78}{0.257}
        & \scalebox{0.78}{0.158} & \scalebox{0.78}{0.276}\\
        
        & \scalebox{0.78}{50\%}
        & \first{\scalebox{0.78}{0.047}} & \first{\scalebox{0.78}{0.142}}
        & \second{\scalebox{0.78}{0.059}} & \second{\scalebox{0.78}{0.158}}
        & \third{\scalebox{0.78}{0.060}} & \third{\scalebox{0.78}{0.162}}
        & \scalebox{0.78}{0.073} & \scalebox{0.78}{0.174}
        & \scalebox{0.78}{0.602} & \scalebox{0.78}{0.572}
        & \scalebox{0.78}{0.232} & \scalebox{0.78}{0.341}
        & \scalebox{0.78}{0.065} & \scalebox{0.78}{0.170}
        & \scalebox{0.78}{0.068} & \scalebox{0.78}{0.173}
        & \scalebox{0.78}{0.369} & \scalebox{0.78}{0.472}
        & \scalebox{0.78}{0.316} & \scalebox{0.78}{0.419}
        & \scalebox{0.78}{0.136} & \scalebox{0.78}{0.268}
        & \scalebox{0.78}{0.183} & \scalebox{0.78}{0.299}\\
        
        \toprule
        
        \multicolumn{2}{c}{\scalebox{0.78}{\avgwins}} &
        \multicolumn{2}{c|}{\first{52.1\%}} &
        \multicolumn{2}{c|}{\second{35.4\%}}  &
        \multicolumn{2}{c|}{\third{18.8\%}} &
        \multicolumn{2}{c|}{0\%} &
        \multicolumn{2}{c|}{0\%} &
        \multicolumn{2}{c|}{0\%} &
        \multicolumn{2}{c|}{0\%} &
        \multicolumn{2}{c|}{0\%} &
        \multicolumn{2}{c|}{0\%} &
        \multicolumn{2}{c|}{0\%} &
        \multicolumn{2}{c|}{0\%} &
        \multicolumn{2}{c}{0\%} \\
        \bottomrule
        
      \end{tabular}
      \end{small}
      \end{threeparttable}
      \label{tab:ds_imputation}
    }
    \vspace{-5mm}
\end{table*}

